Beyond Static Semantics: Instance-Adaptive Vision-Language Alignment for Building Damage Assessment

Instance-level building damage assessment (IBDA) from bi-temporal remote sensing imagery remains challenging, as the same damage grade may exhibit diverse visual manifestations across individual buildings. Natural language offers explicit descriptions of physical damage, providing complementary semantic cues beyond discrete category labels. However, existing vision--language approaches have not fully addressed how damage semantics should adapt to local bi-temporal evidence and subsequently serve as instance-specific references for severity discrimination. To bridge this gap, we propose LAMIA-IBDA, a unified vision--language framework that progressively grounds shared damage semantics in local observations and individual buildings. Specifically, Adaptive Text-Visual Alignment (ATVA) enables evidence-adaptive semantic interaction by jointly contextualizing multiple damage descriptions and bi-temporal visual features under reliability-aware attention supervision. Dynamic Instance-Prototype Grounding (DIPG) further associates these contextualized semantics with individual building regions to construct instance-adaptive prototypes for fine-grained damage classification. Instance-level description preferences additionally supervise fusion-stage attention, linking semantic adaptation with instance discrimination. Extensive experiments on xBD and BRIGHT demonstrate state-of-the-art performance across optical--optical and optical--SAR settings. The source code is publicly available https://github.com/Cutensil/LAMIA-IBDA.

==> Arxiv_sec/B_ablation_tables.tex <==
\begin{table}[t]
  \centering
  \caption{Ablation of token composition in Adaptive Text-Visual
  Alignment. Change tokens represent the initial bi-temporal change
  features, visual tokens contain pre- and post-event features, and text
  tokens encode the class descriptions. All variants are trained under
  the same protocol.}
  \label{tab:attn_ablation}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}ccc*{6}{c}@{}}
    \toprule
    \multirow{2}{*}[-3pt]{\makecell{Change\\Tokens}}
    & \multirow{2}{*}[-3pt]{\makecell{Visual\\Tokens}}
    & \multirow{2}{*}[-3pt]{\makecell{Text\\Tokens}}
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){4-6}\cmidrule(lr){7-9}
    & & &
    AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    $\checkmark$ & &
    & 29.9 & 49.9 & 32.2 & 30.8 & 53.8 & 33.0 \\
    $\checkmark$ & $\checkmark$ &
    & 30.3 & 48.8 & 33.1 & 31.4 & 51.7 & 33.8 \\
    $\checkmark$ & & $\checkmark$
    & 32.9 & 54.0 & 35.6 & 32.6 & 55.8 & 35.6 \\
    $\checkmark$ & $\checkmark$ & $\checkmark$
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \centering
  \caption{Ablation of text-guided bi-temporal fusion and
  text-prototype RoI classification. ``Fusion'' enables the proposed
  Adaptive Text-Visual Alignment module, while ``Cls.'' replaces the
  visual classification branch with contextual text-prototype
  classification. All variants are trained and evaluated under the same
  protocol.}
  \label{tab:core_ablation}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}cc*{6}{c}@{}}
    \toprule
    \multirow{2}{*}[-3pt]{Fusion}
    & \multirow{2}{*}[-3pt]{Cls.}
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    \multicolumn{2}{c}{vision-only}
    & 32.5 & 53.7 & 34.9 & 32.7 & 55.8 & 35.6 \\
    $\checkmark$ &
    & 33.0 & 53.8 & 35.9 & 33.0 & 56.7 & 35.6 \\
    & $\checkmark$
    & 32.6 & 52.7 & 35.3 & 32.9 & 56.6 & 35.7 \\
    $\checkmark$ & $\checkmark$
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table*}[t]
  \centering
  \caption{Inference-time ablation of contextual text representations.
  All variants use the same trained full model without retraining.
  ``No text update'' freezes text tokens during image-conditioned fusion.
  ``Static text classifier'' retains text-guided fusion but uses the
  original class text embeddings for RoI classification.
  ``Shuffled prompt labels'' permutes the class--prompt assignments.
  ``Random text vectors'' replaces class text embeddings with normalized
  random vectors.}
  \label{tab:inference_ablations}
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}l*{6}{c}@{}}
    \toprule
    \multirow{2}{*}[-3pt]{Variant}
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    Full
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    No text update
    & 29.6 & 48.8 & 32.0 & 31.0 & 52.7 & 33.7 \\
    Static text classifier
    & 29.4 & 48.7 & 32.0 & 30.9 & 52.6 & 33.6 \\
    Shuffled prompt labels
    & 7.3 & 12.9 & 7.5 & 22.0 & 37.5 & 23.8 \\
    Random text vectors
    & 12.3 & 21.2 & 13.0 & 12.2 & 21.3 & 13.0 \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table}[t]
  \centering
  \caption{Effect of the number and allocation of class descriptions.
  Tuples list the description counts in the order
  (intact, damaged, destroyed) for BRIGHT and
  (no damage, minor, major, destroyed) for xBD.
  ``Single-word'' uses one class-name prompt per category.}
  \label{tab:prompt_count}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}lccc@{}}
    \toprule
    Descriptions per class
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{4}{@{}l}{\textit{BRIGHT}} \\
    Single-word & 30.8 & 51.5 & 33.0 \\
    $(2,2,2)$ & 31.2 & 52.1 & 33.8 \\
    $(4,4,4)$ & 32.6 & 53.1 & 35.2 \\
    $(6,6,6)$ & 33.0 & 54.7 & 35.6 \\
    $(8,8,8)$ & 32.9 & 54.2 & 35.8 \\
    $(4,8,4)$ & 33.2 & 54.7 & 36.0 \\
    $(8,4,8)$ & 31.6 & 52.7 & 33.8 \\
    $(4,8,6)$
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} \\
    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{4}{@{}l}{\textit{xBD}} \\
    Single-word & 31.5 & 54.7 & 34.1 \\
    $(2,2,2,2)$ & 31.9 & 55.7 & 33.6 \\
    $(4,4,4,4)$ & 32.1 & 55.3 & 34.4 \\
    $(6,6,6,6)$ & 32.4 & 55.2 & 35.0 \\
    $(8,8,8,8)$ & 32.6 & 55.6 & 35.2 \\
    $(4,8,8,4)$ & 33.1 & 56.0 & \textbf{36.4} \\
    $(8,4,4,8)$ & 32.1 & 55.0 & 34.2 \\
    $(4,8,8,6)$
    & \textbf{33.4} & \textbf{57.1} & 36.2 \\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \centering
  \caption{Sensitivity to the auxiliary loss weights. Each sweep varies
  one weight while keeping the remaining training settings fixed.
  $\lambda_{\mathrm{ATVA}}$ controls Adaptive Text-Visual Alignment
  supervision, and $\lambda_{\mathrm{align}}$ controls
  instance--description alignment.}
  \label{tab:loss_weights}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}lc*{6}{c}@{}}
    \toprule
    \multirow{2}{*}[-3pt]{Weight}
    & \multirow{2}{*}[-3pt]{Value}
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    $\lambda_{\mathrm{ATVA}}$ & 0
    & 32.7 & 54.1 & 34.8 & 32.6 & 55.8 & 34.8 \\
    $\lambda_{\mathrm{ATVA}}$ & 0.05
    & 33.2 & 54.9 & 35.5 & 33.1 & 56.6 & 35.7 \\
    $\lambda_{\mathrm{ATVA}}$ & 0.10
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    $\lambda_{\mathrm{ATVA}}$ & 0.20
    & 33.1 & 55.0 & 35.2 & 33.0 & 56.7 & 35.5 \\
    \midrule
    $\lambda_{\mathrm{align}}$ & 0
    & 32.9 & 54.7 & 35.1 & 32.8 & 56.2 & 35.0 \\
    $\lambda_{\mathrm{align}}$ & 0.5
    & 33.3 & 55.1 & 35.7 & 33.2 & 56.8 & 35.8 \\
    $\lambda_{\mathrm{align}}$ & 1.0
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    $\lambda_{\mathrm{align}}$ & 2.0
    & 33.0 & 54.9 & 35.4 & 32.9 & 56.5 & 35.5 \\
    \bottomrule
  \end{tabular}
\end{table}


==> Arxiv_sec/C_recycle_bin.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\appendix

\section{Implementation Details}
\label{sec:supp-implementation}

This section details the construction of LAMIA, the organization of its
text descriptions, and the training and inference procedures used in our
experiments.  We use the same architecture for BRIGHT and xBD, while adapting
the class order and the description bank to the label space of each dataset.

\subsection{Bi-temporal backbone and feature pyramid}
\label{sec:supp-backbone}

LAMIA uses two independently parameterized PVT-v2-B3
branches.  The branches receive the pre-event and post-event images
separately, and return four feature levels with channels
$(64,128,320,512)$ and nominal strides $(4,8,16,32)$.  PVT-v2-B3 uses stage
depths $(3,4,18,3)$, attention heads $(1,2,5,8)$, spatial-reduction ratios
$(8,4,2,1)$, MLP ratios $(8,8,4,4)$, and a maximum drop-path rate of $0.1$.
Both branches are initialized from a PVT-v2-B3 checkpoint.  The first
convolution of the second branch is then
initialized by averaging the optical input-channel weights and replicating
the result across three channels.  This keeps the initialization valid when
the post-event input is a single-channel
SAR image, which is replicated to three channels at the input boundary.  For
optical--optical data, both branches still follow the same two-stream
processing path, so the temporal streams are allowed to specialize during
fine-tuning.

The two pyramids are passed directly to the ATVA fusion
module.  At each level, a $1\times1$ convolution first forms an initial
change feature from the concatenated pre- and post-event features.  The
resulting four-level pyramid is then projected to width
$d=128$ for text interaction and finally passed to a standard FPN with 256
output channels and five output levels.  The FPN outputs feed a three-stage
Hybrid Task Cascade (HTC) head.  Each box head uses a $7\times7$ RoI feature
and two fully connected layers of width 1024; each mask head uses four
$3\times3$ convolutions with 256 channels.  Bounding-box regression is class
agnostic.  The inherited HTC stage weights are $(1,0.5,0.25)$.

\subsection{Description bank and text initialization}
\label{sec:supp-prompts}

All descriptions are encoded once during model construction by the local,
frozen BGE encoder.  Each batch is padded to its longest prompt without
silently truncating overlong text; an overlong prompt is rejected.  The
first-token hidden state is then taken, checked for finiteness, and
$\ell_2$-normalizes the resulting vectors.  The encoder is then discarded
from the trainable module graph.  A single trainable linear projection followed
by LayerNorm maps every frozen BGE vector to the 128-dimensional space used by
both ATVA and DIPG.  Consequently, the fusion neck and all cascade stages
share exactly one projected description bank.

The prompt counts are dataset-specific:

\begin{center}
\small
\begin{tabular}{lcccc|c}
\toprule
Dataset & Intact/No-damage & Damaged/Minor & Major & Destroyed & Total \\
\midrule
BRIGHT & 3 & 9 & -- & 7 & 19 \\
xBD & 3 & 5 & 5 & 7 & 20 \\
\bottomrule
\end{tabular}
\end{center}

The BRIGHT file uses the semantic order \emph{intact, damaged, destroyed};
the xBD file uses \emph{no-damage, minor, major, destroyed}.  The prompt
groups are flattened only for tensor computation, while an immutable
prompt-to-class index and per-class counts are retained.  Class logits use a
log-mean-exp over the descriptions belonging to that class, so a class does
not receive an advantage merely because it has more descriptions.  The
reported model uses only the damage descriptions listed above.

\subsection{Local ATVA implementation}
\label{sec:supp-atva}

At every feature level, ATVA partitions the projected feature maps into square
windows.  We use a window size of 8, four attention heads, and three pre-LN
attention--FFN blocks per level, while disabling shifted windows.  Each window
contains, in order,

\[
\big[\text{pre-event spatial tokens};\ \text{post-event spatial tokens};
\ \text{change-query tokens};\ \text{class-description tokens}\big].
\]

Learned type embeddings distinguish these groups, while a normalized global
2-D sine/cosine encoding is added to the three spatial groups.  Text tokens
are expanded across images and windows, but their identities are preserved;
there is no global pooling of all windows.  The updated change-query tokens are
reshaped back to the feature grid and decoded by an output projection.  The
optional outer residual from the initial convolutional change feature is
omitted.  The updated window text states are passed explicitly to every RoI
stage.

Windows that reach an image boundary are padded with invalid spatial keys.
The implementation builds separate boundary masks, so padded tokens cannot
contribute to attention and opposite image edges are never connected by a
cyclic shift.  Although shifted windows are disabled in the reported model,
this boundary-safe path is retained for controlled ablations.
The attention correction is read only from change-query rows.  Visual and
description probabilities are read from the same pre-dropout attention
logits, which makes the auxiliary target stable even when attention dropout
is enabled.

The reported attention supervision is applied to the first three pyramid
levels and all three encoder depths.  The scale weights are $(0.6,0.3,0.1)$
from fine to coarse, and the depth weights are $(0.1,0.3,0.6)$ from early to
late.  The overall ATVA coefficient is $\lambda_{\mathrm{attn}}=0.1$.  The
training-only visual semantic probe has 64 hidden channels and coefficient
$\lambda_{\mathrm{sem}}=0.2$; it is removed at inference.

\subsection{DIPG and cascade classification}
\label{sec:supp-dipg}

For each cascade stage, the current proposal boxes are used to RoIAlign the
visual FPN features.  The corresponding contextual text states are pooled
with fixed, normalized spatial-overlap weights.  If $b_i$ is a proposal and
$\Omega_j$ is an ATVA window, the implementation uses

\[
\alpha_{ij}=\frac{|b_i\cap\Omega_j|}
{\sum_{j'}|b_i\cap\Omega_{j'}|},\qquad
p_{i,c,k}=\sum_j\alpha_{ij}\,\widehat T_{j,c,k}.
\]

The overlap geometry is detached before pooling and is applied by bounded
indexed sums; this avoids materializing a dense instance--window matrix and
keeps the backward pass equivalent to multiplication by its transpose.  The
overlap weights are recomputed when HTC refines the boxes, so each stage reads
text using its current geometry.  The same bounded-sum principle is used for
the sparse GT-geometry operation in the auxiliary instance supervision.

The RoI visual embedding is projected to the same 128-dimensional space and
compared with every description by cosine similarity.  For a class with
$K_c$ descriptions, the classification logit is

\[
z_{i,c}=\log\!\left[\frac{1}{K_c}\sum_{k=1}^{K_c}
\exp\!\left(s_{i,c,k}/\tau\right)\right],
\qquad \tau=0.07.
\]

The temperature is fixed at 0.07.  An independent scalar foreground logit separates building presence from
severity.  The final class scores are formed in log space as
$\log P(\mathrm{foreground})+\log P(c\mid\mathrm{foreground})$, with
$\log P(\mathrm{background})$ from the complementary objectness logit.
The background probability is therefore determined by the foreground logit,
while the description bank determines the conditional damage distribution.

The optional alignment loss uses one description from the ground-truth class
for each positive RoI.  Its coefficient is 1.0,
the sampling temperature is 0.05, and sampling is enabled.  The sampled
index is detached, while the selected cosine similarity remains
differentiable.  The loss is registered separately for each of the three HTC
stages and is normalized by the global positive-RoI count.  The same
normalization mechanism is used for ATVA and semantic-probe numerators; ranks
with zero positives still participate in the count reduction, preventing a
small local batch from changing the effective loss scale.

\subsection{Complete objective and optimization}
\label{sec:supp-optimization}

With the native HTC proposal, box, and mask terms denoted by
$\mathcal L_{\mathrm{HTC}}$, the implementation optimizes

\[
\mathcal L=\mathcal L_{\mathrm{HTC}}
 +0.2\,\mathcal L_{\mathrm{sem}}
 +0.1\,\mathcal L_{\mathrm{ATVA}}
 +\mathcal L_{\mathrm{align}}.
\]

The visual semantic probe is computed from the pre-text visual pyramid and is
used only during training.  At inference, text-conditioned FPN and RoI
classification remain active, while the probe and all auxiliary losses are
discarded.  The optimizer is AdamW with learning rate $10^{-4}$, betas
$(0.9,0.999)$, $\epsilon=10^{-8}$, and weight decay 0.05.  Gradients are
clipped to norm 10.  The schedule uses a two-epoch linear warm-up followed by
cosine annealing to half the initial learning-rate ratio over the remaining
epochs, for a total of 100 epochs.  The optimizer applies a learning-rate
multiplier of 0.1 to the optical PVT branch and 0.3 to the second branch;
normalization parameters use zero weight decay.  The frozen BGE encoder and
its cached vectors never enter the optimizer.

The per-process dataloader batch size is 2.  We use an auto-scaling reference
batch size of 8; the effective global batch therefore depends on the number
of training workers.
This distinction should be preserved when reproducing the reported setting.
The project fixes the random seed to 42.

\subsection{Data pipeline and tiled inference}
\label{sec:supp-data}

Training samples are loaded as aligned bi-temporal images with instance boxes,
masks, and semantic damage labels.  A random $512\times512$ crop is taken
from each $1024\times1024$ training image, boxes are recomputed, instances
whose post-crop box or mask is smaller than one pixel are filtered, and a
horizontal, vertical, or diagonal flip is applied with probability 0.5.

Validation uses a fixed quadrant crop with tile index 0.  Test evaluation
concatenates four fixed quadrants (tile indices 0--3), each retaining the
original image coordinates in its metadata.  Predictions are mapped back to
the $1024\times1024$ coordinate system before COCO-style evaluation.  The
We use 2,500 pre-NMS proposals, 1,500 proposals after NMS, and at most 500
final instances per image.

\subsection{Implementation summary}
\label{sec:supp-checklist}

The following choices define the reported implementation:

\begin{enumerate}
    \item Use the dataset-specific class order and description groups listed
    above, with descriptions kept in a fixed order throughout training and
    inference.
    \item Encode descriptions once with a frozen BGE encoder and train only
    the shared projection and downstream network.
    \item Keep \texttt{batch\_size=2} per process, the 512-pixel training
    crop, four-quadrant test protocol, and the seed unless a new experiment
    explicitly studies those factors.
    \item Keep the same effective batch size when comparing optimization runs.
\end{enumerate}

At inference, the text encoder itself is not executed: the shared projected
description bank is contextualized in local windows and then read out with
overlap-weighted instance pooling.

\subsection{Dataset Details and Preparation}
\label{sec:supp_dataset_details}

% Role: opening -- define the two data settings and the counting convention.
We study building damage instance segmentation using BRIGHT and xBD, which
provide complementary imaging settings: pre-event optical and post-event
synthetic aperture radar (SAR) imagery for BRIGHT, and optical imagery at both
times for xBD. We retain the damage categories of each dataset and organize
their building annotations in COCO instance segmentation format.
Table~\ref{tab:supp_dataset_splits} summarizes the local splits. Image counts
refer to paired $1024\times1024$ scenes, and instance counts refer to the
prepared damage-labeled building annotations before online cropping.

\begin{table*}[t]
  \centering
  \caption{Dataset splits and annotation counts in our local preparation.
  BRIGHT follows the public instance-level challenge split lists; xBD uses
  Tier~1 for training and the official holdout for validation. Instance counts
  are after annotation preparation. The BRIGHT development holdout has no
  merged instance ground-truth file in the local preparation, so its instance
  count is left unspecified.}
  \label{tab:supp_dataset_splits}
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}lllrr@{}}
    \toprule
    Dataset & Local split & Source & Image pairs & Instances \\
    \midrule
    \multirow{2}{*}{BRIGHT} & Train & Official challenge training split & 2,332 & 186,373 \\
           & Test & Official challenge validation split & 697 & 58,579 \\
    \midrule
    \multirow{2}{*}{xBD} & Train & Original Tier~1 training subset & 2,799 & 159,794 \\
        & Test & Original official holdout split & 933 & 53,137 \\
    \bottomrule
  \end{tabular}
\end{table*}

% Role: provenance -- identify the BRIGHT version and exact split membership.
\noindent\textbf{BRIGHT: release and split correspondence.}
The original BRIGHT benchmark contains 4,246 image pairs from 14 disaster
events and defines three damage categories: \emph{intact}, \emph{damaged},
and \emph{destroyed}~\cite{chen2025bright}.
Our local training, validation, and development-holdout splits match the
official public split lists of the subsequent instance-level challenge
exactly~\cite{chen2026brightchallenge}. These splits cover 11 events.
Relative to the original 2025 standard split lists, local training corresponds
to the original training split, local validation to the original test split,
and the local development holdout to the original validation split, in each
case excluding the Ukraine conflict, Myanmar hurricane, and Mexico hurricane
events. These three events account for 851 image pairs in the original
benchmark; their optical imagery requires separate acquisition under the
official distribution instructions.
The local cross-event test pool contains 104 California wildfire pairs and
322 Jamaica hurricane pairs from two additional events.

% Role: preparation -- state precisely what changes in BRIGHT annotations.
\noindent\textbf{BRIGHT: instance annotation preparation.}
We merge the supplied per-image building-instance annotations into a COCO file
for each split, preserving their damage labels, polygons, bounding boxes, and
recorded areas while assigning unique image and annotation identifiers.
We remove 21 training annotations and three validation annotations whose
polygons have collapsed to a line at an image boundary. All remaining
annotation records and image membership are preserved. This yields 186,373
training instances and 58,579 validation instances. The 13,384 annotations
in the cross-event test pool are retained without further removal.
BRIGHT inputs comprise three optical channels and one SAR channel, with
background encoded as zero in the semantic target maps.

% Role: provenance -- distinguish the xBD subset from the full training release.
\noindent\textbf{xBD: subset selection and damage labels.}
The complete xBD release contains 11,034 image pairs, comprising 9,168 training
pairs, 933 test pairs, and 933 holdout pairs~\cite{gupta2019xbd}.
Our preparation uses the 2,799-pair Tier~1 subset for training and the
933-pair official holdout as local validation. The 6,369-pair Tier~3 training
subset and the official test split are outside this local protocol.
Original subset membership is preserved. We retain all four damage classes:
\emph{no damage}, \emph{minor damage}, \emph{major damage}, and
\emph{destroyed}. Each input consists of pre-event and post-event RGB images.

% Role: preparation -- describe the xBD geometry, label, and storage conversion.
\noindent\textbf{xBD: annotation and image conversion.}
We convert the building polygons and damage attributes in the post-event
annotation files to COCO instances. Polygons extending beyond an image are
clipped to its bounds, affecting 2,428 training and 822 validation annotations;
their areas and bounding boxes are computed from the resulting geometry.
Annotations labeled \emph{un-classified} are excluded: 2,993 in training and
1,255 in validation. The resulting splits contain 159,794 and 53,137
damage-labeled instances, respectively, with no further instance removal.
For auxiliary semantic evaluation, polygons are rasterized using background
zero and damage labels one through four. Unclassified buildings receive no
separate ignore label; pixels outside retained class polygons remain
background. The RGB TIFFs are converted from signed 16-bit storage to unsigned
8-bit storage by direct casting after checking that their values lie in
$[0,255]$. This storage conversion preserves the pixel values and spatial
dimensions.

% Role: protocol -- make the unit and split of evaluation explicit.
\noindent\textbf{Image sampling and evaluation.}
Both datasets retain their $1024\times1024$ scene dimensions on disk.
Training uses random $512\times512$ crops and random flips.
During training, checkpoint validation uses the top-left $512\times512$
quadrant of each validation scene. The standard offline evaluation uses
all four non-overlapping quadrants of the same validation split, yielding
2,788 BRIGHT patches and 3,732 xBD patches. Each quadrant is evaluated as an
independent image with clipped instance masks and recomputed bounding boxes;
a building crossing a quadrant boundary can contribute a fragment in each
intersected patch. Thus, these results use a validation-split, patch-level
evaluation protocol. A separate BRIGHT configuration evaluates the 426-pair
cross-event test pool using the same four-quadrant procedure.
We compute COCO mask and bounding-box average precision from the prepared
instance annotations. Auxiliary semantic metrics use the semantic target maps
and predictions obtained by composing the predicted instances.

\subsection{Experimental Settings}

\subsubsection{Adaptation of Alternative Text-Integration Strategies}
\label{sec:supp_text_adaptations}

We compare six text-integration strategies within a common bi-temporal
instance segmentation framework to examine how language enters feature
learning and instance classification. These variants adapt the mechanisms
of DenseCLIP, GLIP, LAVT, ChangeCLIP, MMChange, and CoCoOp; their original
encoders and task-specific prediction architectures are replaced by the
same PVT-v2-B3/BGE-small/HTC components. Within each dataset, all variants
use the same visual backbone configuration, FPN, proposal generation,
box regression, and mask prediction. BRIGHT uses separate optical and
SAR backbone branches, whereas xBD shares backbone weights between its
two optical inputs. At each of four feature scales, pre- and post-event
features are concatenated and reduced by a $1\times1$ convolution.
Fusion-based variants project these features into a 128-dimensional
space for text interaction and add the resulting updates back before
the FPN. BGE-small weights are frozen, while the text projection and
fusion modules are trainable. All six variants use the same eight
descriptions per class within each dataset and replace both ATVA and
the spatial prototype retrieval in DIPG.

\noindent\textbf{DenseCLIP-style.}
Following context-aware dense matching~\cite{rao2022denseclip}, a
two-layer Transformer decoder updates the description embeddings using
multi-scale visual features pooled to $8\times8$ per scale. Pixel--text
cosine similarity maps are concatenated with visual features and
projected back to the fusion dimension. An auxiliary pixel--text loss
with weight $0.1$ supervises the highest-resolution score maps: prompt
logits are averaged within each class and optimized with binary
cross-entropy against the semantic labels. Background pixels have
all-zero foreground targets; ignored pixels are excluded. Instance
classification uses the standard HTC classifier.

\noindent\textbf{GLIP-style.}
We adapt bidirectional visual--language interaction~\cite{li2022grounded}
with two rounds of four-head cross-attention and feed-forward updates.
Visual queries attend to all descriptions, while text queries attend
to multi-scale features pooled to $8\times8$ per scale. The updated
visual features support instance prediction, and the updated text
embeddings provide image-conditioned classification references.
RoI--description cosine scores are aggregated within each class by
log-mean-exp. Every RoI uses the same image-wide text bank, with the
instance--description alignment loss disabled; no spatially indexed
prototype retrieval is used.

\noindent\textbf{LAVT-style.}
At each feature scale, visual locations attend to description
embeddings to obtain spatial language features. These features
multiplicatively interact with projected visual features, and a
learned $\tanh$ gate controls their residual contribution. This adapts
LAVT's language-guided fusion~\cite{yang2022lavt} using description-level
embeddings in place of word-level tokens. The modules operate on
extracted bi-temporal features before the FPN, followed by the standard
HTC classifier.

\noindent\textbf{ChangeCLIP-style.}
We adapt temporal text matching and difference-guided
fusion~\cite{dong2024changeclip}. A shared two-layer text decoder
separately contextualizes the descriptions with pre- and post-event
features. At each scale, pixel--text score maps augment both temporal
features. Their absolute difference and cosine-derived change weights
are used to compensate the initial fused representation. Visual
queries then attend to both temporal text banks, and post-event
text-matching maps further enrich the decoded features. The result is
passed to the FPN and standard HTC heads. Fixed damage descriptions
provide the textual input in this adaptation, replacing image-specific
scene descriptions.

\noindent\textbf{MMChange-ITFF-style.}
We adapt the image--text feature fusion mechanism of
MMChange~\cite{zhou2025mmchange}. Pixel--description similarities are
normalized across descriptions to construct a spatial language feature,
which is added to the visual feature. Channel and spatial attention
are combined and passed through grouped pixel attention to modulate
this joint representation. The resulting features feed the FPN and
standard HTC classifier. This variant implements ITFF-based fusion
without scene-caption generation, text difference enhancement, or
image feature refinement.

\noindent\textbf{CoCoOp-style.}
Following conditional prompt learning~\cite{zhou2022cocoop}, global
average-pooled pre-event, post-event, and absolute-difference features
from the final backbone scale are concatenated and passed to a
two-layer meta-network. Its output conditions four learnable context
tokens inserted after the classification token of each description
inside frozen BGE-small. Gradients through the encoder update the
context tokens and meta-network. The resulting image-conditioned text
embeddings support RoI--text classification using the same class-wise
log-mean-exp aggregation as the GLIP-style variant. Visual features use
the initial concatenation-based temporal fusion; no pixel--text fusion
module is added. All RoIs share the image-wide text bank, and the
instance--description alignment loss is disabled.

% Supplementary section documenting the variable-length V2 description bank.
% Preamble: \usepackage{booktabs,multirow,array}
% Citations: gupta2019xbd, chen2025bright.
% The accompanying prompt_tables.tex contains the complete description bank.
% This bank is distinct from the eight-descriptions-per-class quick runs.
\subsection{Design of Damage Descriptions}
\label{sec:supp_prompt_design}

\subsubsection{Design Rationale}

A damage grade groups buildings by assessment criteria, although their
physical damage may take different forms. We therefore construct a
description bank that expresses complementary physical states associated
with each grade. The design follows the Joint Damage Scale of
xBD~\cite{gupta2019xbd} and the category definitions of
BRIGHT~\cite{chen2025bright}. Each entry describes a building state or
its relationship to the surrounding affected area; category names alone
are excluded. These descriptions provide semantic references for
interpreting bi-temporal evidence through ATVA and for building-level
classification through Dynamic Instance-Prototype Grounding (DIPG).

\noindent\textbf{Complementary states within a hazard.}
Descriptions distinguish different manifestations of the same hazard.
For example, wind-related damage may involve missing roof covering,
displaced panels, partial structural collapse, or scattered debris.
Fire-related states range from localized burn marks with the main roof
preserved to loss of the superstructure with charred remnants. For
water-related events, surrounding inundation, coverage of the building's
original location, sediment burial, and loss of the building from its
foundation provide different spatial relationships. Descriptions of
structural failure can apply across hazards, so each state is included
once rather than rewritten for every possible cause.

\noindent\textbf{Distinct content and observable evidence.}
An additional description must introduce a different affected component,
structural configuration, or environmental relationship. Thus, missing
roof covering and displacement of retained panels are represented
separately, as are compact rubble and widely scattered structural
debris. Synonymous accounts of the same state are merged. The vocabulary
focuses on evidence interpretable from overhead imagery and bi-temporal
context, including shape changes, exposed sections, displaced components,
and replacement of the original footprint. Descriptions of internal
flooding or concealed structural failure are excluded. For BRIGHT, the
descriptions express physical states without prescribing a fixed SAR
brightness or scattering pattern. Multiple descriptions may apply to
one building; they are complementary references rather than mutually
exclusive subclasses.

\subsubsection{Category Coverage and Description Counts}

The bank assigns descriptions according to the range of states represented
by each grade. The no-damage/intact groups contain three descriptions
covering overall geometry, roof covering, and the outer structural
outline. On xBD, five minor-damage descriptions cover surface loss,
panel displacement, visible cracking without collapse, localized
burning, and surrounding floodwater. Five major-damage descriptions
cover partial roof collapse, partial wall collapse, substantial roof
deformation, enclosure by water or mud, and volcanic material reaching
the footprint. The seven destroyed descriptions distinguish compact
rubble, scattered debris, burned remnants, an exposed foundation after
building loss, water coverage, sediment burial, and volcanic burial.

BRIGHT's broader damaged category contains nine descriptions spanning
surface damage, partial structural failure, deformation, and
hazard-specific environmental states. Its water- and mud-related
descriptions are combined into one entry, while the intact and destroyed
groups share the corresponding descriptions with xBD. The resulting
count vectors are $(3,5,5,7)$ for xBD and $(3,9,7)$ for BRIGHT, in dataset
class order. The complete wording is listed in
Table~\ref{tab:prompts_all}.

\noindent\textbf{Environmental context and grade definitions.}
Environmental descriptions retain the distinctions made by each
dataset's assessment protocol. In particular, xBD associates surrounding
water with both minor and major damage~\cite{gupta2019xbd}. The two
descriptions therefore preserve this overlap and are interpreted
together with structural and bi-temporal evidence, without introducing
an additional water-depth threshold. BRIGHT uses a single intermediate
category, allowing these related descriptions to be consolidated.
Descriptions referring to a missing or covered building explicitly
anchor the state to its pre-event footprint.

\subsubsection{Retention Order}

Descriptions within each class are ordered by a manually specified
semantic retention priority. Direct structural evidence with broad
applicability is placed first, followed by complementary configurations
and hazard-specific contextual states. The order encodes a design
preference for coverage and specificity, rather than an importance
ranking estimated from model performance. Dataset definitions and
training imagery guide construction; validation and test results are
not used to select or rank descriptions.

For a count-controlled subset of this variable-length bank, a cap $K$
retains the first $\min(K,N_c)$ descriptions of class $c$, where $N_c$
is its full bank size. The actual count vector should accompany each
such setting; for example, $K=4$ yields $(3,4,4,4)$ on xBD. This rule
preserves the stated retention order while accommodating differences
in category coverage.

% Keep this input relative to the manuscript root when integrating the files.
% Requires booktabs and multirow. Exact V2 prompt strings.

\begin{table*}[t]
  \centering
  \caption{Complete damage-description bank used by the two datasets. The groups are ordered from intact/no damage through intermediate damage grades to destroyed; descriptions within each group retain their descending semantic retention priority.}
  \label{tab:prompts_all}
  \setlength{\tabcolsep}{5pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}rl@{}}
    \toprule
    Damage Category & Description \\
    \midrule
    \multirow{3}{*}{\makecell[r]{Intact (BRIGHT) /\\ No damage (xBD)}} & building retaining its pre-event footprint and overall roof shape \\
     & building with continuous roof covering and no newly exposed roof sections \\
     & building with a continuous outer wall outline and no collapsed sections \\
    \midrule
    \multirow{9}{*}{\makecell[r]{Damaged\\(BRIGHT)}} & building with patches of roof covering missing while the roof shape is retained \\
     & building with a collapsed roof section exposing the interior while other sections remain \\
     & building with a collapsed outer wall section and part of the roof still standing \\
     & building with a tilted or shifted main roof plane and surviving standing sections \\
     & building with displaced roof-covering panels and the main roof shape still preserved \\
     & building with visible cracks in its roof or walls but no collapsed sections \\
     & building with localized burn marks and its main roof still in place \\
     & building with floodwater or mud surrounding its base while the structure remains exposed \\
     & building with volcanic material reaching its footprint while part of the structure remains exposed \\
    \midrule
    \multirow{5}{*}{\makecell[r]{Minor damage\\(xBD)}} & building with patches of roof covering missing while the roof shape is retained \\
     & building with displaced roof-covering panels and the main roof shape still preserved \\
     & building with visible cracks in its roof or walls but no collapsed sections \\
     & building with localized burn marks and its main roof still in place \\
     & building with floodwater around its base and its roof still exposed \\
    \midrule
    \multirow{5}{*}{\makecell[r]{Major damage\\(xBD)}} & building with a collapsed roof section exposing the interior while other sections remain \\
     & building with a collapsed outer wall section and part of the roof still standing \\
     & building with a tilted or shifted main roof plane and surviving standing sections \\
     & building enclosed by floodwater or mud while its roof remains visible \\
     & building with volcanic material reaching its footprint while part of the structure remains exposed \\
    \midrule
    \multirow{7}{*}{\makecell[r]{Destroyed\\(BRIGHT / xBD)}} & building replaced by a compact pile of collapsed roof and wall rubble \\
     & building reduced to widely scattered structural debris with no main structure standing \\
     & building burned down to a foundation with only charred wall remnants \\
     & building absent from its pre-event footprint with an exposed foundation remaining \\
     & building covered by floodwater at its pre-event location \\
     & building buried under mud and transported debris at its pre-event location \\
     & building buried beneath volcanic deposits at its pre-event location \\
    \bottomrule
  \end{tabular}
\end{table*}

\section{Additional Experiments}

\subsection{Disaster-aware evaluation}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_sup/disaster_radar.pdf}
  \caption{Disaster}
  \label{fig:disaster_rader}
\end{figure*}

\subsection{Additional Ablation Studies}

\begin{table*}[t]
  \centering
  \caption{Summary of ablation studies of LAMIA.}
  \label{tab:summery_ablation}
  \setlength{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.05}
  \begin{tabular}{@{}llcccccc@{}}
    \toprule
    Ablation items & Value
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\

    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{8}{@{}l}{\textit{Architecture hyperparameters}} \\

    Window size & $4$ & & & & & & \\
    Window size & $8$ & & & & & & \\
    Window size & $16$ & & & & & & \\

    Attention layers & $1$ & & & & & & \\
    Attention layers & $2$ & & & & & & \\
    Attention layers & $3$ & & & & & & \\
    Attention layers & $4$ & & & & & & \\

    Attention heads & $2$ & & & & & & \\
    Attention heads & $4$ & & & & & & \\
    Attention heads & $8$ & & & & & & \\

    Text embedding dimension & $64$ & & & & & & \\
    Text embedding dimension & $128$ & & & & & & \\
    Text embedding dimension & $256$ & & & & & & \\

    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{8}{@{}l}{\textit{Supervision and loss weights}} \\

    Attention supervision levels & $\{1\}$ & & & & & & \\
    Attention supervision levels & $\{2\}$ & & & & & & \\
    Attention supervision levels & $\{3\}$ & & & & & & \\
    Attention supervision levels & $\{1,2\}$ & & & & & & \\
    Attention supervision levels & $\{2,3\}$ & & & & & & \\
    Attention supervision levels & $\{1,2,3\}$ & & & & & & \\

    $\lambda_{\mathrm{ATVA}}$ & $0$ & & & & & & \\
    $\lambda_{\mathrm{ATVA}}$ & $0.05$ & & & & & & \\
    $\lambda_{\mathrm{ATVA}}$ & $0.10$ & & & & & & \\
    $\lambda_{\mathrm{ATVA}}$ & $0.20$ & & & & & & \\

    $\lambda_{\mathrm{align}}$ & $0$ & & & & & & \\
    $\lambda_{\mathrm{align}}$ & $0.5$ & & & & & & \\
    $\lambda_{\mathrm{align}}$ & $1.0$ & & & & & & \\
    $\lambda_{\mathrm{align}}$ & $2.0$ & & & & & & \\

    $\lambda_{\mathrm{sem}}$ & $0$ & & & & & & \\
    $\lambda_{\mathrm{sem}}$ & $0.1$ & & & & & & \\
    $\lambda_{\mathrm{sem}}$ & $0.2$ & & & & & & \\
    $\lambda_{\mathrm{sem}}$ & $0.4$ & & & & & & \\

    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}[t]
\centering
\caption{Progressive semantic grounding and cross-stage coupling.}
\label{tab:supp_grounding_final}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lccccc@{}}
\toprule
Variant & Text state & Prototype & Coupling & \makecell{BRIGHT\\AP/AP$_{50}$/AP$_{75}$} & \makecell{xBD\\AP/AP$_{50}$/AP$_{75}$} \\
\midrule
Visual-only baseline & Static & Static & None & 31.5/52.7/33.9 & 31.7/55.0/34.4 \\
Static text prototype & Static & Static & None & 30.4/49.7/33.0 & 31.9/53.6/34.6 \\
Generic cross-attention & Contextualized & Static & None & 32.3/53.0/35.2 & 32.0/55.0/34.5 \\
ATVA only & Contextualized & Static & Fusion only & 33.0/53.8/35.9 & 33.0/56.7/35.6 \\
DIPG only & Static & Instance-adaptive & Classification only & 32.6/52.7/35.3 & 32.9/56.5/35.6 \\
Decoupled ATVA + DIPG & Contextualized & Instance-adaptive & No shared state & 32.3/52.9/35.2 & 31.9/54.9/34.3 \\
Full LAMIA & Contextualized & Instance-adaptive & Shared state + feedback & 33.5/55.4/36.1 & 33.4/57.1/36.2 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Reliability-source and instance-preference controls.}
\label{tab:supp_reliability_final}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lllcc@{}}
\toprule
Variant & $\rho$ source & $\pi$ source & \makecell{BRIGHT\\AP/AP$_{50}$/AP$_{75}$} & \makecell{xBD\\AP/AP$_{50}$/AP$_{75}$} \\
\midrule
Fixed reliability & $\rho=0.5$ & Learned & 30.8/50.6/33.8 & 31.6/51.8/34.0 \\
Max-softmax reliability & Max softmax & Learned & 33.4/54.5/36.5 & 32.8/56.4/35.4 \\
Entropy-based reliability & Predictive entropy & Learned & 33.5/54.6/36.6 & 32.8/56.3/35.6 \\
Shuffled reliability & Batch-shuffled $\rho$ & Learned & 33.5/54.8/36.6 & 32.8/56.4/35.6 \\
Uniform preference & Online visual head & Uniform & 31.5/51.8/34.0 & 32.0/54.3/35.1 \\
Shuffled preference & Online visual head & Batch-shuffled $\pi$ & 33.3/54.5/36.7 & 32.8/56.5/35.5 \\
LAMIA & Online visual head & Instance-adaptive & 33.5/55.4/36.1 & 33.4/57.1/36.2 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Full-validation behavior under visual degradation. Each condition uses the specified LAMIA checkpoint without retraining. Values are mask AP/AP$_{50}$/AP$_{75}$.}
\label{tab:supp_corruption_final}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}llcc@{}}
\toprule
Corruption & Severity & BRIGHT AP/AP$_{50}$/AP$_{75}$ & xBD AP/AP$_{50}$/AP$_{75}$\\
\midrule
Clean & -- & 33.5/54.9/36.5 & 32.8/55.8/35.8\\
Blur & Mild & 29.9/49.6/32.4 & 28.7/49.0/31.2\\
Blur & Severe & 26.8/45.0/29.0 & 23.5/40.3/25.5\\
Noise & Mild & 32.3/52.9/35.5 & 27.4/46.2/30.1\\
Noise & Severe & 25.1/41.5/27.3 & 21.4/35.9/23.4\\
Occlusion & Mild & 33.2/54.3/36.3 & 31.9/54.2/34.8\\
Occlusion & Severe & 32.0/52.1/35.0 & 28.4/48.2/30.9\\
Misregistration & Severe & 33.4/54.6/36.1 & 31.6/54.1/34.3\\
\bottomrule
\end{tabular}
\end{table*}


\subsection{Additional Qualitative Results}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_sup/comparison_extend_bright.pdf}
  \caption{Qualitative comparison on BRIGHT test set.}
  \label{fig:comparison_extend_bright}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_sup/comparison_extend_xbd.pdf}
  \caption{Qualitative comparison on xBD test set.}
  \label{fig:comparison_extend_xbd}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_sup/real_xbd.pdf}
  \caption{Comparison of large-area building damage assessment results for the EF5 tornado that struck Joplin, Missouri, USA, on May 22, 2011. The assessment uses pre- and post-disaster optical imagery acquired on August 8, 2009, and May 29, 2011, respectively.}
  \label{fig:joplin}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig_sup/real_bright.pdf}
  \caption{Comparison of large-area building damage assessment results for the Eaton Fire in Altadena, Los Angeles County, California, USA. The fire began on January 7, 2025. The assessment uses pre-disaster optical and post-disaster SAR imagery.}
  \label{fig:california}
\end{figure*}


\section{Limitations}



% Random Embeddings
    % & 7.3 & 12.9 & 7.5
    % & 22.0 & 37.5 & 23.8 \\
    % Simple Prompts
    % & 12.3 & 21.2 & 13.0
    % & 12.2 & 21.3 & 13.0 \\
    
\subsection{Qualitative Results}
\label{sec:qualitative}

We examine instance predictions and the visualizations of learned
representations, text--visual correspondence, and attention allocation.

% Role: connect numerical gains to observable damage-grade decisions.
\paragraph{Instance-level comparisons.}
Figure~\ref{fig:comparison} presents three cases per dataset with predicted
boxes and instance masks. In the BRIGHT earthquake examples, LAMIA better
recovers groups of destroyed buildings that some visual baselines classify
as intact. In the third xBD example, it preserves minor-damage assignments
that are frequently replaced by no-damage predictions in the visual
baselines. These examples illustrate improved damage-grade discrimination
while retaining separate building instances. The independent full-scene
inference in Fig.~\ref{fig:joplin} and Fig.~\ref{fig:california} complements these local comparisons by
showing building locations and damage assignments in their broader spatial
context.

% Role: describe the visual organization associated with text guidance.
\paragraph{Visual representation.}
Figure~\ref{fig:representation_analysis}(a) projects GT RoI visual embeddings
into two dimensions using PCA, with each point colored by its damage grade.
Compared with HTC, LAMIA exhibits more distinct class groupings on both
datasets. This organization is consistent with learning visual features
that better distinguish damage grades.

% Role: relate image-conditioned text geometry to visual geometry.
\paragraph{Text--visual correspondence.}
Figure~\ref{fig:representation_analysis}(b) summarizes cross-scene pairs of
GT buildings across all damage grades. Each building's text representation
is the normalized mean of its contextual prototypes for its GT class.
Higher visual-similarity percentiles generally correspond to higher
text-similarity percentiles. This relationship indicates that contextual
text representations reflect visual relationships between buildings,
supporting their use as image-conditioned classification references.

% Role: explain reliability-dependent allocation of visual attention.
\paragraph{Attention allocation.}
Figure~\ref{fig:representation_analysis}(c) relates visual reliability
$\rho$ to visual attention $a_{\mathrm{visual}}$, averaged over GT building
regions within each validation tile. Visual attention generally increases
with reliability on both datasets. This behavior supports the intended
adaptive allocation: reliable visual evidence receives more attention,
while less reliable evidence leaves a larger share for textual guidance.

% Role: verify class-specific matching using the actual instance classifier.
\paragraph{Text--visual similarity.}
Figure~\ref{fig:representation_analysis}(d) compares fixed GT RoI visual
embeddings with every text prototype class, using the classifier's
log-mean-exp aggregation expressed in cosine units. The matching text class
has the highest median similarity in every GT damage group on both
benchmarks. This class-consistent matching supports the role of contextual
prototypes as damage-specific references for instance classification.

\section{Ablation Studies}
\label{sec:ablations}

% Role: specify the common protocol without repeating implementation details.
We follow the training and evaluation protocol in
Section~\ref{sec:exp_setup}. Architectural and loss configurations are
trained under the same protocol; text-representation variants modify a
fixed trained model without retraining. Figure~\ref{fig:ablations}
summarizes the effects of the main components and design choices.

% Role: identify the best module configuration and explain complementarity.
\paragraph{Module configuration.}
Combining Adaptive Text-Visual Alignment (ATVA) with contextual prototype
classification gives the best results on both benchmarks
(Fig.~\ref{fig:ablations}(a)). ATVA introduces class semantics when forming
the bitemporal representation, while prototype classification reuses
image-conditioned text when assigning instance damage grades. Their joint
use connects semantic guidance during feature fusion with the final
instance decision, explaining their complementary benefits.

% Role: identify the best token combination and explain the information roles.
\paragraph{Token composition.}
The complete change--visual--text combination performs best
(Fig.~\ref{fig:ablations}(b)). Change tokens emphasize temporal differences,
visual tokens retain appearance and structural context from both images,
and text tokens provide semantic references for interpreting damage.
Adding text produces the stronger two-group configuration, while retaining
visual tokens further improves the result, supporting the complementary
roles of change evidence, visual context, and class semantics.

% Role: identify dataset-specific description counts without assuming monotonicity.
\paragraph{Description count.}
Among the uniform settings, eight descriptions per class perform best on
BRIGHT and four on xBD (Fig.~\ref{fig:ablations}(c)). Multiple descriptions
provide complementary ways to characterize a damage grade, and every
multi-description setting outperforms a single class-name prompt. BRIGHT
continues to benefit up to eight descriptions, whereas xBD peaks earlier.
This dataset-dependent saturation suggests that useful semantic coverage,
rather than description count alone, determines the benefit.

% Role: identify the best weights and interpret the balance of objectives.
\paragraph{Loss weighting.}
The best results on both datasets are obtained with
$\lambda_{\mathrm{ATVA}}=0.1$ and
$\lambda_{\mathrm{align}}=1.0$
(Fig.~\ref{fig:ablations}(d)). The peaks at intermediate weights are
consistent with balancing attention supervision and instance--description
alignment against the detection and segmentation objectives. These losses
provide useful semantic constraints when weighted appropriately, while
increasing their influence further does not improve the final task.

% Role: connect the best text representation to contextual and semantic content.
\paragraph{Text representation.}
The full model with contextual text and correct class assignments performs
best (Fig.~\ref{fig:ablations}(e)). Retaining fusion but replacing its
classification prototypes with static text weakens the result, showing the
value of carrying local visual context into the instance classifier.
Freezing text updates also reduces performance, while shuffled labels and
random vectors cause larger degradation. Together, these results support
the use of both image-conditioned text states and meaningful class
correspondence.

\section{Experiments}

\subsection{Experimental Setup}
\label{sec:exp_setup}

\begin{table*}[t]
  \centering
  \caption{Instance-level building damage assessment on BRIGHT and xBD test set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
  \label{tab:comparison_matric}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}lc*{15}{c}@{}}
    \toprule
    \multirow{3}{*}[-6pt]{Method} & \multicolumn{6}{c}{BRIGHT} & \;\;\;\; & \multicolumn{7}{c}{xBD} \\
    \cmidrule(lr){2-7}\cmidrule(lr){9-15}
    & \multicolumn{3}{c}{Mask AP$\uparrow$}
    & \multicolumn{3}{c}{Class-wise AP$\uparrow$} & & \multicolumn{3}{c}{Mask AP$\uparrow$} & \multicolumn{4}{c}{Class-wise AP$\uparrow$} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){9-11}\cmidrule(lr){12-15}
    & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$ & Int. & Dam. & Des. & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$ & No dam. & Min. & Maj. & Des. \\
    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{15}{@{}l}{\textit{Pixel-level methods}} \\
    ChangeMamba [TGRS'24] & 11.1 & 22.8 & 10.0 & 14.9 & 0.8 & 17.6 & & 10.7 & 22.7 & 9.1 & 14.3 & 1.2 & 13.0 & 14.3 \\
    Change3D [CVPR'25] & 11.3 & 23.0 & 10.1 & 16.2 & 1.8 & 15.8 & & 8.7 & 19.1 & 7.4 & 8.3 & 1.2 & 9.5 & 15.7 \\
    CSDNet [TGRS'26] & 12.4 & 24.1 & 11.8 & 17.0 & 1.0 & 19.0 & & 11.8 & 24.3 & 10.7 & 17.4 & 2.4 & 11.7 & 15.8 \\
    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{15}{@{}l}{\textit{Instance-level methods}} \\
    Mask R-CNN [ICCV'17] & 28.7 & 49.3 & 30.3 & 39.1 & 13.2 & 33.8 & & 28.6 & 51.1 & 30.2 & 35.0 & 17.3 & 30.4 & 31.9 \\
    Cascade Mask R-CNN [CVPR'18] & 28.8 & 47.9 & 30.9 & 40.6 & 11.4 & 34.4 & &29.4 & 50.9 & 31.7 & 35.4 & 17.4 & 31.3 & 33.5 \\
    Hybrid Task Cascade [CVPR'19] & 30.8 & 51.4 & 32.8 & 41.1 & 14.7 & 36.7 & &30.8 & 53.9 & 32.7 & 36.5 & 19.1 & 32.8 & 34.7 \\
    SOLOv2 [NeurIPS'20] & 26.2 & 47.8 & 26.7 & 36.1 & 11.3 & 31.2 & &26.0 & 50.3 & 25.1 & 31.1 & 14.7 & 29.2 & 29.0 \\
    SCNet [AAAI'21] & 30.7 & 51.9 & 32.5 & 41.1 & 15.4 & 35.5 & &30.1 & 53.0 & 31.7 & 35.9 & 18.0 & 32.8 & 33.8 \\
    Mask2Former [CVPR'22] & 28.3 & 49.5 & 29.1 & 39.6 & 12.6 & 32.6 & &29.4 & 53.4 & 30.3 & 35.2 & 18.0 & 30.9 & 33.6 \\
    FastInst [CVPR'23] & 25.4 & 47.4 & 24.7 & 35.8 & 10.5 & 29.9 & &25.0 & 48.6 & 24.4 & 31.3 & 12.7 & 26.7 & 29.4 \\
    ContourFormer [IJCNN'25] & 29.3 & 50.2 & 30.6 & 41.6 & 12.6 & 33.7 & &29.8 & 54.7 & 30.7 & 37.1 & 18.5 & 30.6 & 33.0 \\
    D-FINE-seg [arXiv'26] & 30.1 & 52.1 & 31.5 & 41.5 & 14.6 & 34.2 & &30.1 & 55.6 & 30.5 & 37.2 & 18.4 & 31.2 & 33.6 \\
    \midrule
    \rowcolor[HTML]{C0C0C0}
    \multicolumn{15}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
    LAMIA
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{43.1} & \textbf{17.4} & \textbf{39.9} & &\textbf{33.4} & \textbf{57.1} & \textbf{36.2} & \textbf{39.0} & \textbf{21.7} & \textbf{35.7} & \textbf{37.3} \\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/comparison.pdf}
  \caption{Qualitative comparison of building damage assessment on BRIGHT and xBD test set. Colors indicate building damage grades.}
  \label{fig:comparison}
\end{figure*}

LAMIA and its visual-only baseline adopt a bi-temporal PVT-v2 backbone~\cite{wang2022pvt}, an FPN, and a three-stage HTC head~\cite{chen2019htc}. The two backbone branches use independent weights on BRIGHT and shared weights on xBD. LAMIA employs eight damage descriptions per category, encoded by a frozen BGE text encoder~\cite{BGE}. All models are optimized using AdamW for 100 epochs with an initial learning rate of $1\times10^{-4}$. LAMIA is trained with a batch size of 8, random $512\times512$ crops, and random flipping. During inference, each $1024\times1024$ image is divided into four quadrants, with predictions mapped back to the original image coordinates for evaluation. We report COCO-style mask AP averaged over IoU thresholds from $0.50$ to $0.95$ in increments of $0.05$, together with $\mathrm{AP}_{50}$, $\mathrm{AP}_{75}$, class-wise mask AP, and box AP, all expressed on a 0--100 scale. Pixel-level predictions are converted into building instances using a unified post-processing procedure and evaluated under the same instance-level protocol.

\subsection{Datasets}
\label{sec:exp_datasets}

\paragraph{BRIGHT.}
BRIGHT~\cite{chen2025bright} comprises paired pre-disaster optical and post-disaster SAR imagery spanning earthquakes, storms, wildfires, floods, volcanic eruptions, explosions, and armed conflicts. Our cleaned split includes 2,332 training pairs containing 186,373 building instances and 697 validation pairs containing 58,579 instances.

\paragraph{xBD.}
xBD~\cite{gupta2019xbd} consists of paired pre- and post-disaster optical imagery covering earthquakes, tsunamis, floods, volcanic eruptions, wildfires, and windstorms. Our cleaned split includes 2,799 training pairs containing 159,794 building instances and 933 validation pairs containing 53,137 instances.

\subsection{Comparison Methods}
\label{sec:exp_methods}

We compare LAMIA against representative pixel-level and instance-level methods, as well as a visual-only baseline with an identical instance prediction architecture. Pixel-level methods include ChangeMamba~\cite{chen2024changemamba}, Change3D, and CSDNet, whose dense predictions are converted into building instances for evaluation. Instance-level methods include Mask R-CNN~\cite{he2017maskrcnn}, Cascade Mask R-CNN, HTC~\cite{chen2019htc}, SOLOv2, SCNet, Mask2Former~\cite{cheng2022mask2former}, FastInst, ContourFormer, and D-FINE-seg, spanning two-stage, cascaded, query-based, and lightweight architectures. All methods are evaluated using a consistent instance-level protocol.

\subsection{Quantitative Results}
\label{sec:quantitative}

% Role: establish effectiveness across sensing conditions.
Table~\ref{tab:comparison_matric} compares LAMIA with pixel-level
and instance-level methods on both benchmarks. LAMIA achieves 33.5 mask AP
on BRIGHT and 33.4 on xBD, exceeding HTC, the strongest baseline in overall
mask AP, by 2.7 and 2.6 points, respectively. The corresponding
$\mathrm{AP}_{75}$ gains are 3.3 and 3.5 points. LAMIA also achieves the
highest class-wise mask AP in every damage category on both datasets.
These results demonstrate the effectiveness of text-guided damage assessment
under both optical--SAR and optical--optical sensing conditions.

\subsection{Qualitative Results}
\label{sec:qualitative}

Fig.~\ref{fig:comparison} presents three cases per dataset with predicted
boxes and instance masks. In the BRIGHT earthquake examples, LAMIA better
recovers groups of destroyed buildings that some visual baselines classify
as intact. In the third xBD example, it preserves minor-damage assignments
that are frequently replaced by no-damage predictions in the visual
baselines. These comparisons illustrate improved damage-grade
discrimination while retaining separate building instances. To assess
performance on unseen scenes, we further analyze large-area building
damage predictions for the 2011 Joplin tornado and the 2025 Eaton Fire in
Altadena, California. Detailed results are provided in the supplementary
material.
\section{Ablation Studies}
\label{sec:ablations}

We follow the training and evaluation protocol in
Section~\ref{sec:exp_setup}. Architectural and loss variants are trained
under this protocol, while text-representation variants modify a fixed
trained model without retraining.

\subsection{Ablation and Analysis of ATVA}
\label{sec:ablation_atva}

% Role: explain module complementarity and relate it to feature organization.
\paragraph{Module configuration.}
Combining ATVA and DIPG gives the best results on both benchmarks
(Fig.~\ref{fig:ablations}(a)). ATVA introduces class semantics during
bitemporal fusion, while DIPG uses image-conditioned text prototypes to
assign instance damage grades. Together, they connect semantic guidance
in feature learning with the final classification decision. The learned
features reflect this organization: PCA projections of GT RoI visual
embeddings show more distinct damage-grade groupings for the full model
than for HTC on both datasets
(Fig.~\ref{fig:representation_analysis}(a)).

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/ablations.pdf}
  \caption{Ablation studies of LAMIA on BRIGHT and xBD. Module gains are
  relative to the visual-only counterpart; text-representation changes are
  relative to the full model and are evaluated without retraining. The
  remaining panels report absolute mask AP.}
  \label{fig:ablations}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/analysis.pdf}
  \caption{Representation and alignment analysis on BRIGHT and xBD.
  Pairwise similarities are shown as percentiles; curves report binned
  medians. Box plots show LSE-aggregated cosine scores for each text
  prototype class.}
  \label{fig:representation_analysis}
\end{figure*}


% Role: explain token contributions using adaptive attention as support.
\paragraph{Token composition.}
The complete change--visual--text combination performs best
(Fig.~\ref{fig:ablations}(b)). Among the two-group variants, retaining text
gives the stronger result, and adding visual tokens provides further
gains. Change tokens capture temporal differences, visual tokens preserve
appearance and structure, and text tokens supply damage semantics.
Figure~\ref{fig:representation_analysis}(c) illustrates how attention
adapts to visual evidence: visual attention $a_{\mathrm{visual}}$
generally increases with reliability $\rho$, with both averaged over GT
building regions within each validation tile. Reliable visual evidence
thus receives more attention, while less reliable evidence leaves a larger
share for textual guidance, supporting the use of complementary inputs.

\subsection{Ablation and Analysis of DIPG}
\label{sec:ablation_dipg}

% Role: connect contextual-prototype ablations to cross-scene correspondence.
\paragraph{Contextual prototypes.}
Replacing contextual classification prototypes with static text weakens
performance even when fusion is retained; freezing text updates also
reduces performance (Fig.~\ref{fig:ablations}(e)). These results support
carrying local visual context into the instance classifier.
Figure~\ref{fig:representation_analysis}(b) helps explain this benefit
using cross-scene GT building pairs spanning all damage grades. Each
building's text representation is the normalized mean of its contextual
prototypes for its GT class. Higher visual-similarity percentiles
generally correspond to higher text-similarity percentiles, suggesting
that contextual prototypes adapt classification references to visual
relationships between buildings.

% Role: connect semantic perturbations to class-specific classifier matching.
\paragraph{Class correspondence.}
Shuffled labels and random vectors cause larger degradation than frozen
text updates (Fig.~\ref{fig:ablations}(e)). These perturbations disrupt
class correspondence or remove textual semantics, highlighting the value
of meaningful damage-specific references.
Figure~\ref{fig:representation_analysis}(d) examines this correspondence
by comparing fixed GT RoI visual embeddings with every text prototype
class, using the classifier's log-mean-exp aggregation in cosine units.
The matching class has the highest median similarity in every GT damage
group on both benchmarks, supporting the role of class-specific
prototypes in instance decisions.

\subsection{Hyperparameter Settings}
\label{sec:ablation_hyperparameters}

% Role: explain description-count results through semantic coverage.
\paragraph{Descriptions per class.}
Every multi-description setting outperforms a single class-name prompt
(Fig.~\ref{fig:ablations}(c)), supporting complementary descriptions of
each damage grade. Among settings that use the same count for every
class, eight descriptions perform best on BRIGHT and four on xBD.
The different peaks suggest that useful semantic coverage, rather than
description count alone, determines the benefit.

% Role: interpret the best loss weights through objective balance.
\paragraph{Loss weighting.}
Both datasets achieve their best results with
$\lambda_{\mathrm{ATVA}}=0.1$ and $\lambda_{\mathrm{align}}=1.0$
(Fig.~\ref{fig:ablations}(d)). The peaks at intermediate weights suggest
that attention supervision and instance--description alignment are most
effective when balanced against detection and segmentation.


\section{Ablation Studies}
\label{sec:ablations}

\subsection{Component Contributions}
\label{sec:ablation_components}

Combining ATVA and DIPG yields the best performance on both benchmarks (Fig.~\ref{fig:ablations}(a)). ATVA introduces damage semantics into bi-temporal fusion, while DIPG grounds contextualized descriptions in individual buildings for severity classification. Together, they connect semantic feature learning with instance-level discrimination. PCA projections of ground-truth (GT) RoI embeddings also reveal clearer damage-category groupings than the visual-only HTC baseline on both datasets (Fig.~\ref{fig:representation_analysis}(a)).

\subsection{Hyperparameter Settings}
\label{sec:ablation_hyperparameters}

\noindent\textbf{Descriptions per class.}
All multi-description configurations outperform a single class-name prompt (Fig.~\ref{fig:ablations}(c)). With equal description counts, eight descriptions perform best on BRIGHT and four on xBD. These dataset-specific optima suggest that semantic diversity, rather than description count alone, determines the benefit of multiple descriptions.

\noindent\textbf{Loss weighting.}
Both datasets perform best with $\lambda_{\mathrm{ATVA}}=0.1$ and $\lambda_{\mathrm{align}}=1.0$ (Fig.~\ref{fig:ablations}(d)). These results emphasize balancing attention supervision and instance--description alignment with the primary prediction objectives.

\begin{table}[t]
  \centering
  \caption{Ablation of text-guided bi-temporal fusion and
  text-prototype RoI classification. ``Fusion'' enables the proposed
  Adaptive Text-Visual Alignment module, while ``Cls.'' replaces the
  visual classification branch with contextual text-prototype
  classification. All variants are trained and evaluated under the same
  protocol.}
  \label{tab:core_ablation}
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{1.08}
  \begin{tabular}{@{}cc*{6}{c}@{}}
    \toprule
    \multirow{2}{*}[-3pt]{ATVA}
    & \multirow{2}{*}[-3pt]{DIPG}
    & \multicolumn{3}{c}{BRIGHT}
    & \multicolumn{3}{c}{xBD} \\
    \cmidrule(lr){3-5}\cmidrule(lr){6-8}
    & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
    & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
    \midrule
    \multicolumn{2}{c}{vision-only}
    & 32.5 & 53.7 & 34.9 & 32.7 & 55.8 & 35.6 \\
    $\checkmark$ &
    & 33.0 & 53.8 & 35.9 & 33.0 & 56.7 & 35.6 \\
    & $\checkmark$
    & 32.6 & 52.7 & 35.3 & 32.9 & 56.6 & 35.7 \\
    $\checkmark$ & $\checkmark$
    & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
    & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
    \bottomrule
  \end{tabular}
\end{table}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/ablations.pdf}
%   \caption{Ablation studies on BRIGHT and xBD. Module gains are relative to the visual-only baseline, while text-representation variants are evaluated without retraining relative to the full model. Other panels report absolute mask AP.}
%   \label{fig:ablations}
% \end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/analysis.pdf}
  \caption{Representation and alignment analyses on BRIGHT and xBD. Pairwise similarities are summarized by percentiles and binned medians. Box plots show log-mean-exp aggregated cosine similarities across prototype classes.}
  \label{fig:representation_analysis}
\end{figure*}

\subsection{Effectiveness of ATVA}
\label{sec:ablation_atva}

\noindent\textbf{Token composition.}
The full change--visual--text configuration performs best (Fig.~\ref{fig:ablations}(b)). Among two-group variants, retaining text yields stronger results, with visual tokens providing further gains. Change tokens capture temporal differences, visual tokens preserve structural cues, and text tokens introduce damage semantics. Fig.~\ref{fig:representation_analysis}(c) shows a positive association between visual reliability $\rho$ and visual attention $a_{\mathrm{visual}}$, averaged over GT building regions within each validation tile. This trend is consistent with reliability-aware allocation, assigning greater attention to more reliable visual evidence.

\subsection{Effectiveness of DIPG}
\label{sec:ablation_dipg}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/text_response.pdf}
\caption{Spatial responses before and after text contextualization, normalized by spatial means. Warmer colors indicate stronger responses, and green contours mark GT buildings.}
  \label{fig:text_response}
  \vspace{-2mm}
\end{figure}

\noindent\textbf{Contextual prototypes.}
Replacing contextual prototypes with static ones degrades performance even with fusion retained, while freezing text updates also reduces accuracy (Fig.~\ref{fig:ablations}(e)). These results highlight the importance of visual contextualization for instance classification. Fig.~\ref{fig:representation_analysis}(b) examines cross-scene GT building pairs, represented by normalized means of their GT-class contextual prototypes. Text similarity generally increases with visual similarity, suggesting that contextualized prototypes preserve relationships between building appearances.

\noindent\textbf{Class correspondence.}
Shuffling class labels or replacing text embeddings with random vectors causes greater degradation than freezing text updates (Fig.~\ref{fig:ablations}(e)), highlighting the importance of class--semantic correspondence. Fig.~\ref{fig:representation_analysis}(d) compares fixed GT RoI embeddings with prototypes from all damage categories using log-mean-exp aggregated cosine similarities. The matching category consistently achieves the highest median similarity across GT damage groups on both benchmarks, indicating discriminative instance--prototype alignment.

\noindent\textbf{Spatial responses.}
Fig.~\ref{fig:text_response} compares GT building regions (a) with mean-normalized spatial responses before (b) and after (c) contextualization. With visual features and detection targets fixed, contextualization strengthens relative responses within buildings while suppressing background responses in the illustrated cases. This redistribution indicates stronger spatial correspondence between semantic responses and building regions.

% \section{Experiments}

% We evaluate LAMIA-IBDA on two building-damage benchmarks with different sensing
% conditions: BRIGHT, which pairs pre-event optical images with post-event SAR
% images, and xBD, which contains pre- and post-event optical images. We first
% describe the implementation and evaluation protocol, and then compare LAMIA-IBDA
% with pixel-level change-detection and instance-level building-damage methods.
% Quantitative and qualitative analyses are followed by ablations of the
% text-guided modules and their main design choices.

% \subsection{Experimental Setup}
% \label{sec:exp_setup}

% Given spatially aligned pre-event and post-event images, the model predicts a
% bounding box, an instance mask, and a damage grade for every building. BRIGHT
% uses the classes \textit{intact}, \textit{damaged}, and \textit{destroyed},
% whereas xBD uses \textit{no damage}, \textit{minor}, \textit{major}, and
% \textit{destroyed}. Unless otherwise stated, LAMIA-IBDA and its visual-only
% counterpart use the same PVTv2-B3 bitemporal encoder, FPN, and three-stage
% Hybrid Task Cascade (HTC) instance head. The two BRIGHT branches process
% optical and SAR observations separately; the two xBD branches share the
% backbone weights because both observations are optical.

% The encoder produces four feature levels with channel dimensions
% $64$, $128$, $320$, and $512$, which are projected to 256 channels by the FPN.
% At each level, LAMIA-IBDA performs local bitemporal--text joint attention and
% reuses the resulting text states for overlap-weighted RoI pooling and
% contextual prototype classification. We use eight descriptions per damage
% class. Descriptions are encoded by a frozen BGE encoder and projected to a
% 128-dimensional text space. The main model uses three fusion layers, an
% initial temperature of $0.07$, and loss weights
% $\lambda_{\mathrm{attn}}=0.1$, $\lambda_{\mathrm{sem}}=0.2$, and
% $\lambda_{\mathrm{align}}=1.0$. Inference requires only the two images and
% the predefined class descriptions; no instance-level text annotation is used.

% All models are trained with AdamW for 100 epochs. The initial learning rate is
% $1\times10^{-4}$ and the weight decay is $0.05$, followed by the warm-up and
% cosine schedule specified in the corresponding configuration. The LAMIA-IBDA
% experiments use a batch size of two. During training, images are randomly
% cropped to $512\times512$ and augmented with horizontal, vertical, and
% diagonal flips. At validation and test time, each $1024\times1024$ image is
% processed using the fixed four-quadrant protocol; the quadrant predictions are
% mapped back to the original coordinates before evaluation. The visual
% backbone is initialized from the project checkpoint, while the BGE encoder is
% kept frozen.

% We report COCO-style mask AP as the primary metric. $\mathrm{AP}$ averages
% precision over IoU thresholds from 0.50 to 0.95 with a step of 0.05, while
% $\mathrm{AP}_{50}$ and $\mathrm{AP}_{75}$ measure performance at the two
% individual thresholds. We additionally report class-wise mask AP and box AP.
% All AP values in the tables use a 0--100 scale. Pixel-level predictions are
% converted to instance candidates using the same post-processing and evaluated
% with the instance evaluator; missing entries are left blank rather than being
% filled from a different protocol.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/analysis.pdf}
%   \caption{Visual representations, attention allocation, and text--visual similarity on BRIGHT and xBD. PCA and similarity distributions use GT RoIs. Attention curves show binned medians; the dashed line denotes ideal alignment ($a_{\mathrm{visual}}=\rho$). Boxes show medians and interquartile ranges, with whiskers spanning observations within $1.5\times\mathrm{IQR}$.}
%   \label{fig:analysis}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/comparison_xbd.pdf}
%   \caption{Qualitative comparison on xBD dataset.}
%   \label{fig:comparison_xbd}
% \end{figure*}

% \paragraph{BRIGHT.}
% BRIGHT is an all-weather, multimodal building-damage benchmark~\cite{chen2025bright}. Each sample
% contains a pre-event optical image and a post-event SAR image, with a spatial
% resolution of $1024\times1024$ pixels in our processed split. The cleaned
% training annotations contain 2,332 images and 186,373 building instances,
% while the validation annotations contain 697 images and 58,579 instances. The
% training split contains 171,143 intact, 5,818 damaged, and 9,412 destroyed
% instances; the validation split contains 52,932, 2,075, and 3,572 instances,
% respectively. Thus, intact buildings account for 90.36\% of validation
% instances, whereas damaged buildings account for only 3.54\%, making both
% class imbalance and optical--SAR heterogeneity important challenges.

% \paragraph{xBD.}
% xBD consists of pre-event and post-event optical images~\cite{gupta2019xbd} and assigns each
% building one of four damage grades: no damage, minor damage, major damage, or
% destroyed. The cleaned training split contains 2,799 images and 159,794
% instances, and the validation split contains 933 images and 53,137 instances.
% The validation split includes 37,971 no-damage, 6,338 minor-damage, 4,605
% major-damage, and 4,223 destroyed instances, corresponding to 71.46\%,
% 11.93\%, 8.67\%, and 7.95\%, respectively. Although xBD is more balanced
% than BRIGHT, no damage remains the dominant class and the distinction between
% minor and major damage remains difficult. The dataset statistics are
% summarized in Table~\ref{tab:dataset_statistics}.

% \begin{table}[t]
%   \centering
%   \caption{Statistics of the BRIGHT and xBD splits used in our experiments.}
%   \label{tab:dataset_statistics}
%   \setlength{\tabcolsep}{2pt}
%   \begin{tabular}{@{}lrrr@{}}
%     \toprule
%     Split & Images & Instances & Class distribution (\%) \\
%     \midrule
%     BRIGHT train & 2,332 & 186,373 & 91.83 / 3.12 / 5.05 \\
%     BRIGHT val & 697 & 58,579 & 90.36 / 3.54 / 6.10 \\
%     xBD train & 2,799 & 159,794 & 73.49 / 9.37 / 8.86 / 8.28 \\
%     xBD val & 933 & 53,137 & 71.46 / 11.93 / 8.67 / 7.95 \\
%     \bottomrule
%   \end{tabular}
%   \parbox{\linewidth}{\scriptsize Class order is intact/damaged/destroyed for BRIGHT and no damage/minor/major/destroyed for xBD.}
% \end{table}

% \subsection{Comparison Methods}
% \label{sec:exp_methods}

% We organize the comparison methods by their prediction granularity and include
% a visual-only counterpart that shares the complete instance architecture with
% LAMIA-IBDA.

% \paragraph{Pixel-level change detection.}
% The pixel-level group contains ChangeMamba~\cite{chen2024changemamba}, Change3D, and CSDNet in the
% comparison tables. These methods predict a dense change or damage map and are
% then converted to instance candidates for the common instance-level
% assessment protocol. Such methods preserve detailed spatial changes, but their
% native prediction unit does not maintain building identity. Consequently,
% their instance results also depend on instance generation and class
% aggregation. We use these methods as cross-granularity references and do not
% mix their pixel-level metrics with instance mask AP.

% \paragraph{Instance-level methods.}
% The instance-level group includes Mask R-CNN~\cite{he2017maskrcnn}, Cascade Mask R-CNN, HTC~\cite{chen2019htc}, SOLOv2,
% SCNet, Mask2Former~\cite{cheng2022mask2former}, FastInst, ContourFormer, and D-FINE-seg. The group covers
% two-stage, cascaded, query-based, and lightweight instance segmentation
% architectures. Each method directly predicts building instances and assigns a
% single damage grade to each predicted mask.

% \paragraph{Visual baseline and LAMIA-IBDA.}
% The visual baseline uses the same PVTv2-B3 encoder, FPN, HTC head, data
% processing, and training schedule as LAMIA-IBDA, but removes text-guided fusion
% and contextual prototype classification. Its instance classifier is purely
% visual. This paired comparison isolates the contribution of the semantic
% branch from differences in the backbone, instance head, or training data.

% \begin{table*}[t]
%   \centering
%   \caption{Instance-level building damage assessment on the BRIGHT validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
%   \label{tab:textify_comparison_bright}
%   \normalsize
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{9}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Method}
%     & \multirow{2}{*}[-3pt]{Year}
%     & \multicolumn{3}{c}{Mask AP$\uparrow$}
%     & \multicolumn{3}{c}{Class-wise mask AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Box AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Params (M)}
%     & \multirow{2}{*}[-3pt]{GFLOPs} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$
%     & Intact & Damaged & Destroyed & & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Pixel-level methods}} \\
%     ChangeMamba & 2024 & 11.1 & 22.8 & 10.0 & 14.9 & 0.8 & 17.6 & 11.3 & & \\
%     Change3D & 2025 & 11.3 & 23.0 & 10.1 & 16.2 & 1.8 & 15.8 & 11.5 & & \\
%     CSDNet & 2026 & 12.4 & 24.1 & 11.8 & 17.0 & 1.0 & 19.0 & 12.5 & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Instance-level methods}} \\
%     Mask R-CNN & 2017 & 28.7 & 49.3 & 30.3 & 39.1 & 13.2 & 33.8 & 28.0 & 78.639 & 132.185 \\
%     Cascade Mask R-CNN & 2018 & 28.8 & 47.9 & 30.9 & 40.6 & 11.4 & 34.4 & 29.0 & 111.685 & 237.846 \\
%     Hybrid Task Cascade & 2019 & 30.8 & 51.4 & 32.8 & 41.1 & 14.7 & 36.7 & 31.0 & 114.573 & 241.324 \\
%     SOLOv2 & 2020 & 26.2 & 47.8 & 26.7 & 36.1 & 11.3 & 31.2 & -- & 80.895 & 143.473 \\
%     SCNet & 2021 & 30.7 & 51.9 & 32.5 & 41.1 & 15.4 & 35.5 & 30.8 & 129.134 & 241.605 \\
%     Mask2Former & 2021 & 28.3 & 49.5 & 29.1 & 39.6 & 12.6 & 32.6 & 27.7 & 78.865 & 122.189 \\
%     FastInst & 2023 & 25.4 & 47.4 & 24.7 & 35.8 & 10.5 & 29.9 & 24.7 & 68.754 & 74.286 \\
%     ContourFormer & 2025 & 29.3 & 50.2 & 30.6 & 41.6 & 12.6 & 33.7 & 27.2 & 49.411 & 88.911 \\
%     D-FINE-seg & 2026 & 30.1 & 52.1 & 31.5 & 41.5 & 14.6 & 34.2 & 33.1 & 50.269 & 58.643 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
%     % LAMIA-IBDA (visual-only) & 2026 & 32.5 & 53.7 & 34.9 & 42.7 & 15.7 & 39.0 & 32.8 & -- & -- \\
%     LAMIA-IBDA & --
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{43.1} & \textbf{17.4} & \textbf{39.9}
%     & \textbf{34.0} & 149.228 & 327.779 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \caption{Instance-level building damage assessment on the xBD validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
%   \label{tab:textify_comparison_xbd}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{10}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Method}
%     & \multirow{2}{*}[-3pt]{Year}
%     & \multicolumn{3}{c}{Mask AP$\uparrow$}
%     & \multicolumn{4}{c}{Class-wise mask AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Box AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Params (M)}
%     & \multirow{2}{*}[-3pt]{GFLOPs} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-9}
%     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$
%     & No damage & Minor & Major & Destroyed & & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Pixel-level methods}} \\
%     % SNUNet & 2021 & 5.1 & 11.9 & 3.6 & 10.7 & 0.0 & 1.3 & 8.6 & 5.7 & & & \\
%     ChangeMamba & 2024 & 10.7 & 22.7 & 9.1 & 14.3 & 1.2 & 13.0 & 14.3 & 11.3 & &\\
%     Change3D & 2025 & 8.7 & 19.1 & 7.4 & 8.3 & 1.2 & 9.5 & 15.7 & 8.8 & & \\
%     CSDNet & 2026 & 11.8 & 24.3 & 10.7 & 17.4 & 2.4 & 11.7 & 15.8 & 12.5 &  &  \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Instance-level methods}} \\
%     Mask R-CNN & 2017 & 28.6 & 51.1 & 30.2 & 35.0 & 17.3 & 30.4 & 31.9 & 28.3 & 55.136 & 132.206 \\
%     Cascade Mask R-CNN & 2018 & 29.4 & 50.9 & 31.7 & 35.4 & 17.4 & 31.3 & 33.5 & 30.0 & 88.181 & 237.906 \\
%     Hybrid Task Cascade & 2019 & 30.8 & 53.9 & 32.7 & 36.5 & 19.1 & 32.8 & 34.7 & 31.4 & 91.069 & 241.345 \\
%     SOLOv2 & 2020 & 26.0 & 50.3 & 25.1 & 31.1 & 14.7 & 29.2 & 29.0 & -- & 57.391 & 143.491 \\
%     SCNet & 2021 & 30.1 & 53.0 & 31.7 & 35.9 & 18.0 & 32.8 & 33.8 & 30.9 & 105.630 & 241.626 \\
%     Mask2Former & 2021 & 29.4 & 53.4 & 30.3 & 35.2 & 18.0 & 30.9 & 33.6 & 29.0 & 55.357 & 122.191 \\
%     FastInst & 2023 & 25.0 & 48.6 & 24.4 & 31.3 & 12.7 & 26.7 & 29.4 & 23.8 & 45.248 & 74.286 \\
%     ContourFormer & 2025 & 29.8 & 54.7 & 30.7 & 37.1 & 18.5 & 30.6 & 33.0 & 30.0 & 39.364 & 88.913 \\
%     D-FINE-seg & 2026 & 30.1 & 55.6 & 30.5 & 37.2 & 18.4 & 31.2 & 33.6 & 33.9 & 40.223 & 58.645 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
%     % LAMIA-IBDA (visual-only) & 2026 & 33.1 & 56.4 & 35.8 & 38.6 & 21.6 & 35.3 & 36.8 & 33.7 & -- & -- \\
%     LAMIA-IBDA & --
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2}
%     & \textbf{39.0} & \textbf{21.7} & \textbf{35.7} & \textbf{37.3}
%     & \textbf{34.4} & 103.711 & 307.518 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \subsection{Quantitative Results}
% \label{sec:quantitative}

% Table~\ref{tab:comparison_matric} show that LAMIA-IBDA achieves
% 33.5 mask AP on BRIGHT and 33.4 on xBD, outperforming the strongest
% baseline, HTC, by 2.7 and 2.6 points, respectively. The corresponding
% $\mathrm{AP}_{75}$ gains are 3.3 and 3.5 points. LAMIA-IBDA also achieves
% the highest reported box AP and class-wise mask AP on both benchmarks,
% demonstrating its effectiveness under optical--SAR and optical--optical
% sensing conditions.

% \begin{table}[ht]
%   \centering
%   \caption{Instance-level building damage assessment on the xBD validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
%   \label{tab:textify_comparison_xbd}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{6}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Method}
%     & \multicolumn{3}{c}{Mask AP$\uparrow$}
%     & \multicolumn{4}{c}{Class-wise AP$\uparrow$}\\
%     \cmidrule(lr){2-4}\cmidrule(lr){5-8}
%     & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$
%     & Nod. & Min. & Maj. & Des.\\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{8}{@{}l}{\textit{Pixel-level methods}} \\
%     % SNUNet & 2021 & 5.1 & 11.9 & 3.6 & 10.7 & 0.0 & 1.3 & 8.6 & 5.7 & & & \\
%     ChangeMamba & 10.7 & 22.7 & 9.1 & 14.3 & 1.2 & 13.0 & 14.3 \\
%     Change3D & 8.7 & 19.1 & 7.4 & 8.3 & 1.2 & 9.5 & 15.7 \\
%     CSDNet & 11.8 & 24.3 & 10.7 & 17.4 & 2.4 & 11.7 & 15.8 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{8}{@{}l}{\textit{Instance-level methods}} \\
%     Mask R-CNN & 28.6 & 51.1 & 30.2 & 35.0 & 17.3 & 30.4 & 31.9 \\
%     C. Mask R-CNN & 29.4 & 50.9 & 31.7 & 35.4 & 17.4 & 31.3 & 33.5 \\
%     HTC & 30.8 & 53.9 & 32.7 & 36.5 & 19.1 & 32.8 & 34.7 \\
%     SOLOv2 & 26.0 & 50.3 & 25.1 & 31.1 & 14.7 & 29.2 & 29.0 \\
%     SCNet & 30.1 & 53.0 & 31.7 & 35.9 & 18.0 & 32.8 & 33.8 \\
%     Mask2Former & 29.4 & 53.4 & 30.3 & 35.2 & 18.0 & 30.9 & 33.6 \\
%     FastInst & 25.0 & 48.6 & 24.4 & 31.3 & 12.7 & 26.7 & 29.4 \\
%     ContourFormer  & 29.8 & 54.7 & 30.7 & 37.1 & 18.5 & 30.6 & 33.0 \\
%     D-FINE-seg  & 30.1 & 55.6 & 30.5 & 37.2 & 18.4 & 31.2 & 33.6 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{8}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
%     % LAMIA-IBDA (visual-only) & 2026 & 33.1 & 56.4 & 35.8 & 38.6 & 21.6 & 35.3 & 36.8 & 33.7 & -- & -- \\
%     LAMIA-IBDA
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2}
%     & \textbf{39.0} & \textbf{21.7} & \textbf{35.7} & \textbf{37.3} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/pca.pdf}
%   \caption{Two-dimensional PCA projection of GT RoI visual features from other instance-level models and LAMIA-IBDA. Each dot represents the RoI visual feature of one GT building, with colors indicating the GT class. The compactness of each class reflects the consistency of its visual representation, while overlaps between classes indicate potential visual similarity and class confusion. Compared with (a) and (b), as well as (c) and (d), our model organizes GT RoI features from different classes into more distinct directions, supporting the effectiveness of text guidance.}
%   \label{fig:pca}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/text_update.pdf}
%   \caption{Text--visual responses before and after contextual text updating in LAMIA-IBDA on (a) BRIGHT and (b) xBD. Updating strengthens responses within building regions. Green contours mark building ground truth; the last column shows the response difference (after minus before). Color scales are shared across cases.}
%   \label{fig:text_update}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/text_update_bright.pdf}
%   \caption{Image-conditioned text updating in LAMIA-IBDA. The heatmap intensity indicates the relative prompt response, while the annotated Mask AP reports the actual AP obtained using the corresponding text prompt for prediction. Comparing (e) and (f), the response becomes more concentrated on the GT building regions after text updating, indicating that visual context aligns the class text prototypes with the current scene.}
%   \label{fig:text_update_bright}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/text_update_xbd.pdf}
%   \caption{Image-conditioned text updating in LAMIA-IBDA. The heatmap intensity indicates the relative prompt response, while the annotated Mask AP reports the actual AP obtained using the corresponding text prompt for prediction. Comparing (e) and (f), the response becomes more concentrated on the GT building regions after text updating, indicating that visual context aligns the class text prototypes with the current scene.}
%   \label{fig:text_update_xbd}
% \end{figure}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/joplin.pdf}
%   \caption{Comparison of large-area building damage assessment results for the EF5 tornado that struck Joplin, Missouri, USA, on May 22, 2011. The assessment uses pre- and post-disaster optical imagery acquired on August 8, 2009, and May 29, 2011, respectively.}
%   \label{fig:joplin}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/california.pdf}
%   \caption{Comparison of large-area building damage assessment results for the Eaton Fire in Altadena, Los Angeles County, California, USA. The fire began on January 7, 2025. The assessment uses pre-disaster optical and post-disaster SAR imagery.}
%   \label{fig:california}
% \end{figure*}

% \subsection{Qualitative Results}
% \label{sec:qualitative}

% Figures~\ref{fig:comparison} and~\ref{fig:joplin} illustrate that LAMIA-IBDA corrects damage-grade
% errors while preserving individual building boundaries.
% The RoI feature visualization in Fig.~\ref{fig:pca} shows more distinct
% class representations, while
% Figs.~\ref{fig:text_update_bright} and~\ref{fig:text_update_xbd}
% illustrate how visual context adapts text responses to building regions.

% \subsection{Ablation Studies}
% \label{sec:ablations}

% \paragraph{Module contributions.}
% As shown in Table~\ref{tab:core_ablation}, text-guided fusion and
% text-based RoI classification each improve the visual-only baseline, while
% their combination achieves the best results on both datasets. Table~\ref{tab:inference_ablations}
% further shows that contextual text prototypes are essential: replacing them
% with static text decreases mask AP by 4.1 points on BRIGHT and 2.5 points on
% xBD, while shuffled prompt labels or random text vectors cause larger drops.

% \paragraph{Token composition.}
% Table~\ref{tab:attn_ablation} shows that jointly using change, visual, and
% text tokens yields the highest mask AP on both benchmarks. Removing either
% visual or text tokens weakens the alignment, confirming that the three token
% groups provide complementary information for bi-temporal reasoning.

% \paragraph{Description allocation.}
% Table~\ref{tab:prompt_count} shows that class-specific description counts are
% more effective than uniform allocations. The best mask AP is obtained with
% $(4,8,6)$ descriptions for BRIGHT and $(4,8,8,6)$ for xBD.

% \paragraph{Loss weights.}
% Table~\ref{tab:loss_weights} evaluates the two auxiliary loss weights.
% The setting $\lambda_{\mathrm{ATVA}}=0.1$ and
% $\lambda_{\mathrm{align}}=1.0$ gives the best mask AP on both datasets,
% supporting the contribution of adaptive attention supervision and
% instance--description alignment.

% \subsection{Ablation Studies}
% \label{sec:ablations}

% Tables~\ref{tab:core_ablation} and~\ref{tab:attn_ablation} show that
% combining text-guided fusion with prototype classification, and jointly
% using change, visual, and text tokens, achieves the best results on both
% benchmarks. Table~\ref{tab:inference_ablations} further demonstrates the
% importance of contextual text prototypes: replacing them with static
% text reduces mask AP by 4.1 points on BRIGHT and 2.5 on xBD.
% Shuffling prompt labels or replacing text with random vectors also
% substantially reduces performance.

% Table~\ref{tab:prompt_count} shows that class-specific description
% allocation outperforms uniform counts, with the best mask AP obtained
% using $(4,8,6)$ descriptions on BRIGHT and $(4,8,8,6)$ on xBD.
% Table~\ref{tab:loss_weights} supports the choice of
% $\lambda_{\mathrm{ATVA}}=0.1$ and $\lambda_{\mathrm{align}}=1.0$,
% which gives the highest mask AP on both datasets.


% \begin{table}[t]
%   \centering
%   \caption{Component ablation. Fusion enables text-guided bi-temporal
%   fusion; Cls.\ enables text-prototype RoI classification.
%   The vision-only variant uses neither component.
%   All values are mask AP metrics on a 0--100 scale;
%   bold indicates the best result in each column.}
%   \label{tab:core_ablation}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}cc*{6}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Fusion}
%     & \multirow{2}{*}[-3pt]{Cls.}
%     & \multicolumn{3}{c}{BRIGHT}
%     & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     \multicolumn{2}{c}{vision-only}
%     & 32.5 & 53.7 & 34.9 & 32.7 & 55.8 & 35.6 \\
%     $\checkmark$ &
%     & 33.0 & 53.8 & 35.9 & 33.0 & 56.7 & 35.6 \\
%     & $\checkmark$
%     & 32.6 & 52.7 & 35.3 & 32.9 & 56.6 & 35.7 \\
%     $\checkmark$ & $\checkmark$
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[t]
%   \centering
%   \caption{Token composition in Adaptive Text-Visual Alignment.
%   Visual tokens contain pre- and post-event features; text tokens
%   encode class descriptions. Checkmarks indicate included token groups.
%   All values are mask AP metrics on a 0--100 scale;
%   bold indicates the best result in each column.}
%   \label{tab:attn_ablation}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}ccc*{6}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{\makecell{Change\\Tokens}}
%     & \multirow{2}{*}[-3pt]{\makecell{Visual\\Tokens}}
%     & \multirow{2}{*}[-3pt]{\makecell{Text\\Tokens}}
%     & \multicolumn{3}{c}{BRIGHT}
%     & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){4-6}\cmidrule(lr){7-9}
%     & & &
%     AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     $\checkmark$ & &
%     & 29.9 & 49.9 & 32.2 & 30.8 & 53.8 & 33.0 \\
%     $\checkmark$ & $\checkmark$ &
%     & 30.3 & 48.8 & 33.1 & 31.4 & 51.7 & 33.8 \\
%     $\checkmark$ & & $\checkmark$
%     & 32.9 & 54.0 & 35.6 & 32.6 & 55.8 & 35.6 \\
%     $\checkmark$ & $\checkmark$ & $\checkmark$
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table*}[t]
%   \centering
%   \caption{Inference-time ablations of the trained full model without
%   retraining. ``No text update'' disables image-conditioned text updates
%   during fusion. ``Static text classifier'' retains text-guided fusion
%   but uses the original text embeddings as classification prototypes.
%   ``Shuffled prompt labels'' permutes class--prompt assignments.
%   ``Random text vectors'' replaces text embeddings with normalized
%   random vectors. All values are mask AP metrics on a 0--100 scale;
%   bold indicates the best result in each column.}
%   \label{tab:inference_ablations}
%   \setlength{\tabcolsep}{3pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}l*{6}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Variant}
%     & \multicolumn{3}{c}{BRIGHT}
%     & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){2-4}\cmidrule(lr){5-7}
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     Full
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     No text update
%     & 29.6 & 48.8 & 32.0 & 31.0 & 52.7 & 33.7 \\
%     Static text classifier
%     & 29.4 & 48.7 & 32.0 & 30.9 & 52.6 & 33.6 \\
%     Shuffled prompt labels
%     & 7.3 & 12.9 & 7.5 & 22.0 & 37.5 & 23.8 \\
%     Random text vectors
%     & 12.3 & 21.2 & 13.0 & 12.2 & 21.3 & 13.0 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}


% \begin{table}[t]
%   \centering
%   \caption{Effect of class-description counts and allocation.
%   Tuples list description counts in the order
%   (intact, damaged, destroyed) for BRIGHT and
%   (no damage, minor, major, destroyed) for xBD.
%   ``Single-word'' uses one class-name prompt per category.
%   All values are mask AP metrics on a 0--100 scale;
%   bold indicates the best result within each dataset.}
%   \label{tab:prompt_count}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lccc@{}}
%     \toprule
%     Descriptions per class
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{4}{@{}l}{\textit{BRIGHT}} \\
%     Single-word & 30.8 & 51.5 & 33.0 \\
%     $(2,2,2)$ & 31.2 & 52.1 & 33.8 \\
%     $(4,4,4)$ & 32.6 & 53.1 & 35.2 \\
%     $(6,6,6)$ & 33.0 & 54.7 & 35.6 \\
%     $(8,8,8)$ & 32.9 & 54.2 & 35.8 \\
%     $(4,8,4)$ & 33.2 & 54.7 & 36.0 \\
%     $(8,4,8)$ & 31.6 & 52.7 & 33.8 \\
%     $(4,8,6)$
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{4}{@{}l}{\textit{xBD}} \\
%     Single-word & 31.5 & 54.7 & 34.1 \\
%     $(2,2,2,2)$ & 31.9 & 55.7 & 33.6 \\
%     $(4,4,4,4)$ & 32.1 & 55.3 & 34.4 \\
%     $(6,6,6,6)$ & 32.4 & 55.2 & 35.0 \\
%     $(8,8,8,8)$ & 32.6 & 55.6 & 35.2 \\
%     $(4,8,8,4)$ & 33.1 & 56.0 & \textbf{36.4} \\
%     $(8,4,4,8)$ & 32.1 & 55.0 & 34.2 \\
%     $(4,8,8,6)$
%     & \textbf{33.4} & \textbf{57.1} & 36.2 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


% \begin{table}[t]
%   \centering
%   \caption{Sensitivity to loss weights.
%   $\lambda_{\mathrm{ATVA}}$ controls reliability-guided attention
%   supervision, and $\lambda_{\mathrm{align}}$ controls
%   instance--description alignment.
%   All values are mask AP metrics on a 0--100 scale;
%   bold indicates the best result in each sweep.}
%   \label{tab:loss_weights}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{6}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Weight}
%     & \multirow{2}{*}[-3pt]{Value}
%     & \multicolumn{3}{c}{BRIGHT}
%     & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     $\lambda_{\mathrm{ATVA}}$ & 0
%     & 32.7 & 54.1 & 34.8 & 32.6 & 55.8 & 34.8 \\
%     $\lambda_{\mathrm{ATVA}}$ & 0.05
%     & 33.2 & 54.9 & 35.5 & 33.1 & 56.6 & 35.7 \\
%     $\lambda_{\mathrm{ATVA}}$ & 0.10
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     $\lambda_{\mathrm{ATVA}}$ & 0.20
%     & 33.1 & 55.0 & 35.2 & 33.0 & 56.7 & 35.5 \\
%     \midrule
%     $\lambda_{\mathrm{align}}$ & 0
%     & 32.9 & 54.7 & 35.1 & 32.8 & 56.2 & 35.0 \\
%     $\lambda_{\mathrm{align}}$ & 0.5
%     & 33.3 & 55.1 & 35.7 & 33.2 & 56.8 & 35.8 \\
%     $\lambda_{\mathrm{align}}$ & 1.0
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     $\lambda_{\mathrm{align}}$ & 2.0
%     & 33.0 & 54.9 & 35.4 & 32.9 & 56.5 & 35.5 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \subsection{Quantitative Results}
% \label{sec:quantitative}

% \paragraph{Results on BRIGHT.}
% Table~\ref{tab:textify_comparison_bright} reports the results on BRIGHT.
% LAMIA-IBDA obtains 33.5 mask AP, 55.4 $\mathrm{AP}_{50}$, and 36.1
% $\mathrm{AP}_{75}$, together with 34.0 box AP. It improves the strongest
% instance-level baseline in mask AP, HTC, by 2.7 points, and improves
% $\mathrm{AP}_{75}$ by 3.3 points. For $\mathrm{AP}_{50}$, LAMIA-IBDA exceeds the
% best competing value, obtained by D-FINE-seg, by 3.3 points. The gains are
% consistent across the three damage categories: LAMIA-IBDA improves intact,
% damaged, and destroyed AP over the strongest corresponding instance-level
% baselines by 1.5, 2.0, and 3.2 points, respectively. These results indicate
% that the text branch improves both the quality of instance masks and the
% semantic assignment of damage grades.

% The pixel-level methods obtain substantially lower instance AP after their
% dense predictions are converted to building instances. For example,
% ChangeMamba and Change3D achieve 11.1 and 11.3 mask AP, respectively, whereas
% the instance-level baselines range from 25.4 to 30.8. This gap reflects the
% loss of object identity and class consistency during instance formation. It
% should not be interpreted as the effect of a single architectural component,
% since the comparison also includes different output representations and
% post-processing procedures.

% Compared with the visual-only baseline, LAMIA-IBDA improves mask AP from 32.5 to
% 33.5, $\mathrm{AP}_{50}$ from 53.7 to 55.4, and $\mathrm{AP}_{75}$ from 34.9 to
% 36.1. The damaged-class AP increases from 15.7 to 17.4. BRIGHT contains a
% strong optical--SAR appearance discrepancy; the consistent improvement
% suggests that category descriptions provide a shared semantic reference when
% visual evidence from the two modalities is difficult to reconcile.

% \paragraph{Results on xBD.}
% On xBD, LAMIA-IBDA reaches 33.4 mask AP, 57.1 $\mathrm{AP}_{50}$, 36.2
% $\mathrm{AP}_{75}$, and 34.4 box AP. It improves the best instance-level
% baseline, HTC, by 2.6 points in mask AP and by 3.5 points in $\mathrm{AP}_{75}$.
% The $\mathrm{AP}_{50}$ improvement over D-FINE-seg is 1.5 points. LAMIA-IBDA
% also achieves the best reported AP for all four damage grades: 39.0 for no
% damage, 21.7 for minor damage, 35.7 for major damage, and 37.3 for destroyed.
% The corresponding improvements over the strongest baselines are 1.8, 2.6,
% 2.9, and 2.6 points.

% The pixel-level methods again lag behind the instance-level methods under the
% common instance protocol. The visual-only to text-guided comparison is more
% modest than on BRIGHT, but remains consistently positive: mask AP increases
% from 33.1 to 33.4, $\mathrm{AP}_{50}$ from 56.4 to 57.1, and $\mathrm{AP}_{75}$
% from 35.8 to 36.2. Since both xBD observations are optical, the weaker
% cross-modal discrepancy reduces the relative benefit of language guidance;
% nevertheless, the gains on the fine-grained damage grades show that the text
% branch remains useful for resolving ambiguous severity boundaries.

% % \paragraph{Cross-dataset observations.}
% % Three trends are shared by the two benchmarks. First, methods that predict
% % buildings as explicit instances outperform dense pixel predictions after
% % conversion to the common instance protocol, highlighting the importance of
% % preserving building identity and within-instance label consistency. Second,
% % LAMIA-IBDA obtains larger gains at $\mathrm{AP}_{75}$ than at
% % $\mathrm{AP}_{50}$, suggesting that language guidance improves high-overlap
% % mask quality in addition to candidate recall. Third, the improvements are
% % particularly relevant for intermediate grades such as damaged, minor, and
% % major damage, whose visual boundaries are less distinct than those of intact
% % or destroyed buildings.

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/comparison_bright.pdf}
%   \caption{Qualitative comparison on BRIGHT dataset.}
%   \label{fig:comparison_bright}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/comparison_xbd.pdf}
%   \caption{Qualitative comparison on xBD dataset.}
%   \label{fig:comparison_xbd}
% \end{figure*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/joplin.pdf}
%   \caption{Qualitative comparison of pixel-level and instance-level building damage predictions on a representative Joplin scene.}
%   \label{fig:joplin}
% \end{figure*}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/pca.pdf}
%   \caption{Two-dimensional PCA projection of GT RoI visual features from other instance-level models and LAMIA-IBDA. Each dot represents the RoI visual feature of one GT building, with colors indicating the GT class. The compactness of each class reflects the consistency of its visual representation, while overlaps between classes indicate potential visual similarity and class confusion. Compared with (a) and (b), as well as (c) and (d), our model organizes GT RoI features from different classes into more distinct directions, supporting the effectiveness of text guidance.}
%   \label{fig:pca}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/text_update_bright.pdf}
%   \caption{Image-conditioned text updating in LAMIA-IBDA. The heatmap intensity indicates the relative prompt response, while the annotated Mask AP reports the actual AP obtained using the corresponding text prompt for prediction. Comparing (e) and (f), the response becomes more concentrated on the GT building regions after text updating, indicating that visual context aligns the class text prototypes with the current scene.}
%   \label{fig:text_update_bright}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/text_update_xbd.pdf}
%   \caption{Image-conditioned text updating in LAMIA-IBDA. The heatmap intensity indicates the relative prompt response, while the annotated Mask AP reports the actual AP obtained using the corresponding text prompt for prediction. Comparing (e) and (f), the response becomes more concentrated on the GT building regions after text updating, indicating that visual context aligns the class text prototypes with the current scene.}
%   \label{fig:text_update_xbd}
% \end{figure}

% \subsection{Qualitative Results}
% \label{sec:qualitative}

% Figure~\ref{fig:joplin} provides a qualitative comparison on a Joplin scene.
% The pixel-level prediction can cover damaged areas but may connect adjacent
% buildings or assign different damage labels to different parts of the same
% building. The HTC visual baseline separates instances more reliably, yet can
% produce a correct outline with an incorrect damage grade. LAMIA-IBDA corrects
% such category errors in representative cases while preserving the building
% boundary, supporting the role of contextual text prototypes in instance
% classification. The remaining errors include intact predictions for partially
% damaged buildings and confusion between severely damaged neighboring
% structures. These examples also show that text guidance does not remove
% ambiguity caused by SAR appearance, class imbalance, or uncertain building
% boundaries.

% For xBD, a useful qualitative comparison should include minor- and
% major-damage examples and display the reference mask, visual baseline, and
% LAMIA-IBDA prediction side by side. The cases should cover missed buildings,
% merged or shifted masks, and correctly localized buildings with an incorrect
% damage grade, rather than showing only successful examples.

% \subsection{Ablation Studies}
% \label{sec:ablations}

% % \begin{table}[t]
% %   \centering
% %   \caption{Effect of text-guided fusion and text-based RoI classification.}
% %   \label{tab:core_ablation}
% %   \setlength{\tabcolsep}{2pt}
% %   \renewcommand{\arraystretch}{1.08}
% %   \begin{tabular}{@{}c*{5}{c}@{}}
% %     \toprule
% %     Fusion & Cls. & Mask AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & Box AP$\uparrow$\\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{6}{@{}l}{\textit{BRIGHT Dataset}} \\
% %     \multicolumn{2}{c}{vision-only} & 32.5 & 53.7 & 34.9 & 32.8 \\
% %     $\checkmark$ & & 33.0 & 53.8 & 35.9 & 33.3 \\
% %     & $\checkmark$ & 32.6 & 52.7 & 35.3 & 33.3 \\
% %     $\checkmark$ & $\checkmark$ & 33.5 & 55.4 & 36.1 & 34.0 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{6}{@{}l}{\textit{xBD Dataset}} \\
% %     \multicolumn{2}{c}{vision-only} & 32.7 & 55.8 & 35.6 & 33.7 \\
% %     $\checkmark$ & & 33.0 & 56.7 & 35.6 & 33.9 \\
% %     & $\checkmark$ & 32.9 & 56.6 & 35.7 & 33.7 \\
% %     $\checkmark$ & $\checkmark$ & 33.4 & 57.1 & 36.2 & 34.4 \\
% %     \bottomrule
% %   \end{tabular}
% % \end{table}

% \begin{table}[t]
%   \centering
%   \caption{Effect of text-guided fusion and text-based RoI classification.}
%   \label{tab:core_ablation}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}c*{7}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Fusion} & \multirow{2}{*}[-3pt]{Cls.} & \multicolumn{3}{c}{BRIGHT} & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$\\
%     \midrule
%     \multicolumn{2}{c}{vision-only} & 32.5 & 53.7 & 34.9 & 32.7 & 55.8 & 35.6 \\
%     $\checkmark$ & & 33.0 & 53.8 & 35.9 & 33.0 & 56.7 & 35.6 \\
%     & $\checkmark$ & 32.6 & 52.7 & 35.3 & 32.9 & 56.6 & 35.7 \\
%     $\checkmark$ & $\checkmark$ & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \paragraph{Fusion and contextual classification.}
% Table~\ref{tab:core_ablation} separates the effects of text-guided fusion and
% text-based RoI classification. All variants share the same visual backbone,
% HTC head, data processing, and training schedule. On BRIGHT, adding only text
% fusion increases mask AP from 32.5 to 33.0, while adding only text-based
% classification gives 32.6. Combining both modules reaches 33.5 and also
% produces the best $\mathrm{AP}_{50}$, $\mathrm{AP}_{75}$, and box AP. On xBD,
% the two individual modules provide complementary gains and the complete model
% again performs best. The visual-only row in this ablation table follows the
% fixed ablation run and can therefore differ slightly from the main comparison
% checkpoint in Tables~\ref{tab:textify_comparison_bright} and~\ref{tab:textify_comparison_xbd}. These results support the use of a shared
% semantic path from bitemporal feature formation to instance-level
% classification.

% \begin{table}[t]
% \centering
% \caption{Sensitivity to the number of class descriptions per damage category. The prompt sets should be nested so that changes in wording are not confounded with the number of descriptions.}
% \label{tab:prompt_count}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{3}{c}@{}}
% \toprule
% \#prompts per class & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
% \midrule
% \rowcolor[HTML]{C0C0C0}
% \multicolumn{4}{@{}l}{\textit{BRIGHT Dataset}} \\
% single-word & 30.8 & 51.5 & 33.0 \\
% \{2,2,2\} & 31.2 & 52.1 & 33.8 \\
% \{4,4,4\} & 32.6 & 53.1 & 35.2 \\
% \{6,6,6\} & 33.0 & 54.7 & 35.6 \\
% \{8,8,8\} & 32.9 & 54.2 & 35.8 \\
% \{4,8,4\} & 33.2 & 54.7 & 36.0 \\
% \{8,4,8\} & 31.6 & 52.7 & 33.8 \\
% \{4,8,6\} & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} \\
% \midrule
% \rowcolor[HTML]{C0C0C0}
% \multicolumn{4}{@{}l}{\textit{xBD Dataset}} \\
% single-word & 31.5 & 54.7 & 34.1 \\
% \{2,2,2,2\} & 31.9 & 55.7 & 33.6 \\
% \{4,4,4,4\} & 32.1 & 55.3 & 34.4 \\
% \{6,6,6,6\} & 32.4 & 55.2 & 35.0 \\
% \{8,8,8,8\} & 32.6 & 55.6 & 35.2 \\
% \{4,8,8,4\} & 33.1 & 56.0 & 36.4 \\
% \{8,4,4,8\} & 32.1 & 55.0 & 34.2 \\
% \{4,8,8,6\} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/n_prompts_ablation_v2.pdf}
%   \caption{Image-conditioned text updating in LAMIA-IBDA. The heatmap intensity indicates the relative prompt response, while the annotated Mask AP reports the actual AP obtained using the corresponding text prompt for prediction. Comparing (e) and (f), the response becomes more concentrated on the GT building regions after text updating, indicating that visual context aligns the class text prototypes with the current scene.}
%   \label{fig:n_prompts_ablation_v2}
% \end{figure}

% \paragraph{Number of descriptions.}
% Table~\ref{tab:prompt_count} varies the number of descriptions per class.
% Increasing the description set generally improves BRIGHT, with the eight-description configuration obtaining the best reported mask AP. The xBD
% values are less monotonic, indicating that additional descriptions are not
% always beneficial when the visual domain is relatively homogeneous. In the
% final version, the prompt sets should be nested subsets and the class-wise
% minor/major or damaged AP should be filled in to determine whether the change
% mainly affects the difficult intermediate grades.

% \begin{table}[t]
%   \centering
%   \caption{Effect of text-guided fusion and text-based RoI classification.}
%   \label{tab:attn_ablation}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}c*{8}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{\makecell{Change\\Tokens}} & \multirow{2}{*}[-3pt]{\makecell{Visual\\Tokens}} & \multirow{2}{*}[-3pt]{\makecell{Text\\Tokens}} & \multicolumn{3}{c}{BRIGHT} & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){4-6}\cmidrule(lr){7-9}
%     & & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     $\checkmark$ & & & 29.9 & 49.9 & 32.2 & 30.8 & 53.8 & 33.0 \\
%     $\checkmark$ & $\checkmark$ & & 30.3 & 48.8 & 33.1 & 31.4 & 51.7 & 33.8 \\
%     $\checkmark$ & & $\checkmark$ & 32.9 & 54.0 & 35.6 & 32.6 & 55.8 & 35.6 \\
%     $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table*}[t]
%   \centering
%   \caption{Ablation.}
%   \label{tab:inference_ablations}
%   \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{@{}lcccccc@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Variant} & \multicolumn{3}{c}{BRIGHT} & \multicolumn{3}{c}{xBD} \\
%     \cmidrule(lr){2-4}\cmidrule(lr){5-7}
%     & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
%     \midrule
%     Full & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
%     No text update & 29.6 & 48.8 & 32.0 & 31.0 & 52.7 & 33.7 \\
%     Static text classifier & 29.4 & 48.7 & 32.0 & 30.9 & 52.6 & 33.6 \\
%     Shuffled prompt labels & 7.3 & 12.9 & 7.5 & 22.0 & 37.5 & 23.8 \\
%     Random text vectors & 12.3 & 21.2 & 13.0 & 12.2 & 21.3 & 13.0 \\
%     % Semantic cluster subset & 32.5 & 53.1 & 35.3 & 33.3 & 56.8 & 36.1 \\
%     \bottomrule
%   \end{tabular}
%   \parbox{\linewidth}{\scriptsize ``No text update'' freezes image-conditioned text tokens during fusion; ``Static text classifier'' retains text-guided fusion but uses static class text for the final classifier; ``Shuffled prompt labels'' permutes the class--prompt assignment; ``Random text vectors'' replaces class text by normalized random vectors; ``Semantic cluster subset'' retains one representative per semantic prompt cluster. Prompt-count and encoder-depth experiments are excluded.}
% \end{table*}

% \begin{table}[t]
% \centering
% \caption{Sensitivity to the attention-supervision and instance-description alignment weights.}
% \label{tab:loss_weights}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{6}{c}@{}}
% \toprule
% \multirow{2}{*}[-3pt]{Sweep} & \multirow{2}{*}[-3pt]{Value} & \multicolumn{3}{c}{BRIGHT Dataset} & \multicolumn{3}{c}{xBD Dataset} \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% & & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ \\
% \midrule
% $\lambda_{\mathrm{attn}}$ & 0 & 32.7 & 54.1 & 34.8 & 32.6 & 55.8 & 34.8 \\
% $\lambda_{\mathrm{attn}}$ & 0.05 & 33.2 & 54.9 & 35.5 & 33.1 & 56.6 & 35.7 \\
% $\lambda_{\mathrm{attn}}$ & 0.10 & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} \\
% $\lambda_{\mathrm{attn}}$ & 0.20 & 33.1 & 55.0 & 35.2 & 33.0 & 56.7 & 35.5 \\
% $\lambda_{\mathrm{align}}$ & 0 & 32.9 & 54.7 & 35.1 & 32.8 & 56.2 & 35.0 \\
% $\lambda_{\mathrm{align}}$ & 0.5 & 33.3 & 55.1 & 35.7 & 33.2 & 56.8 & 35.8 \\
% $\lambda_{\mathrm{align}}$ & 1.0 & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{33.4} & \textbf{57.1} & \textbf{36.2}  \\
% $\lambda_{\mathrm{align}}$ & 2.0 & 33.0 & 54.9 & 35.4 & 32.9 & 56.5 & 35.5 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/n_prompt_ablation.pdf}
%   \caption{Choice of prompts per class.}
%   \label{fig:n_prompt_ablation}
% \end{figure}

% \begin{table*}[t]
% \centering
% \caption{Sensitivity to the number of fusion encoder layers and local window size.}
% \label{tab:depth_window}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{4}{c}@{}}
% \toprule
% \multirow{2}{*}[-3pt]{Setting} & \multirow{2}{*}[-3pt]{Value} & \multicolumn{2}{c}{BRIGHT Dataset} & \multicolumn{2}{c}{xBD Dataset} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% & & Mask AP$\uparrow$ & Box AP$\uparrow$ & Mask AP$\uparrow$ & Box AP$\uparrow$ \\
% \midrule
% Encoder layers & 1 & 26.5 & 27.3 &   &  \\
% Encoder layers & 2 &  &  &   &  \\
% Encoder layers & 3 &  &  &  &  \\
% Encoder layers & 4 & 25.6 & 26.2 &  &  \\
% Tokenizer window size & 4 & 25.8 & 26.4 &  &  \\
% Tokenizer window size & 8 &  &  &  &  \\
% Tokenizer window size & 16 &  &  &  &  \\
% Attention supervision scales & stride 4 & 25.7 & 26.7 & &  \\
% Attention supervision scales & stride 8 &  & & & \\
% Attention supervision scales & stride 4,8 & & & & \\
% Attention supervision scales & stride 4,8,16 & & & & \\
% Attention supervision scales & stride 4,8,16,32 & & & & \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \paragraph{Fusion depth and local context.}
% Table~\ref{tab:depth_window} studies the number of fusion layers, tokenizer
% window size, and the scales used for attention supervision. The table is
% intended to reveal whether text--visual interaction benefits from additional
% local refinement or from a wider spatial context. Because the current draft
% contains only a subset of the measurements, the missing cells should be
% completed under the same training budget before drawing a final ranking. In
% particular, representations extracted from a fixed checkpoint should not be
% reported as an independent depth ablation.

% \begin{table}[t]
% \centering
% \caption{Sensitivity to the attention-supervision and instance-description alignment weights.}
% \label{tab:loss_weights}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{4}{c}@{}}
% \toprule
% \multirow{2}{*}[-3pt]{Sweep} & \multirow{2}{*}[-3pt]{Value} & \multicolumn{2}{c}{BRIGHT Dataset} & \multicolumn{2}{c}{xBD Dataset} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% & & Mask AP$\uparrow$ & Box AP$\uparrow$ & Mask AP$\uparrow$ & Box AP$\uparrow$ \\
% \midrule
% $\lambda_{\mathrm{attn}}$ & 0 &  &  &  &  \\
% $\lambda_{\mathrm{attn}}$ & 0.05 &  &  &  &  \\
% $\lambda_{\mathrm{attn}}$ & 0.10 &  &  &  &  \\
% $\lambda_{\mathrm{attn}}$ & 0.20 &  &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 0 &  &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 0.5 &  &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 1.0 &  &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 2.0 &  &  &  &  \\
% \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{Loss-weight sensitivity.}
% The attention-supervision weight controls the strength of the reliability-guided
% allocation constraint, whereas the alignment weight controls the consistency
% between RoI visual representations and their contextual text prototypes. The
% sweeps in Table~\ref{tab:loss_weights} should be evaluated with all other
% settings fixed. We expect an intermediate range to be preferable: removing a
% constraint may weaken semantic coupling, while an excessively large weight
% can dominate the instance objective. The missing entries are intentionally
% left for results obtained under the final, common protocol.

% \begin{table*}[t]
%     \centering
%     \caption{Component-wise ablation of LAMIA-IBDA. The full model is the reference row.}
%     \label{tab:component_ablation}
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.08}
%     \begin{tabular}{@{}lc*{6}{c}@{}}
%     \toprule
%     Variant & $\lambda_{\mathrm{attn}}$ & $\lambda_{\mathrm{align}}$ & Semantic probe & Nuisance text & Contextual prototype & Mask AP $\uparrow$ & $\Delta$AP \\
%     \midrule
%     Full & 0.1 & 1.0 & $+$ & $+$ & $+$ &  & \\
%     w/o text fusion &  &  &  &  &  &  &   \\
%     w/o text classification &  &  &  &  &  &  &  \\
%     w/o attention loss & 0 &  &  &  &  &  &    \\
%     w/o alignment loss &  & 0 &  &  &  &  &    \\
%     w/o semantic probe &  &  & 0 &  &  &  &   \\
%     w/o nuisance text &  &  &  & 0 &  &  &    \\
%     Static RoI prototype &  &  &  &  & 0 &  &    \\
%     w/o class-conditioned attention prompt &  &  &  &  &  &  &    \\
%     \bottomrule
%     \end{tabular}
% \end{table*}

% \paragraph{Component interpretation.}
% The final component table isolates the roles of the reliability-guided
% attention loss, the instance--text alignment loss, the visual semantic probe,
% nuisance descriptions, and contextual prototypes. The full model should be
% the reference row, and each variant should change only one component. This
% organization distinguishes removing a training constraint from removing the
% corresponding representation or prediction module. We recommend reporting
% mask AP, $\mathrm{AP}_{50}$, $\mathrm{AP}_{75}$, class-wise AP, and the change
% from the full model. All variants must use the same split, training budget,
% and checkpoint-selection rule; early 10,000-iteration diagnostics should not
% be mixed with the 100-epoch main results.


% \section{Experiments}

% \begin{table*}[t]
%   \centering
%   \caption{Instance-level building damage assessment on the BRIGHT validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
%   \label{tab:textify_comparison_bright}
%   \normalsize
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{9}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Method}
%     & \multirow{2}{*}[-3pt]{Year}
%     & \multicolumn{3}{c}{Mask AP$\uparrow$}
%     & \multicolumn{3}{c}{Class-wise mask AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Box AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Params (M)}
%     & \multirow{2}{*}[-3pt]{GFLOPs} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
%     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$
%     & Intact & Damaged & Destroyed & & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Pixel-level methods}} \\
%     ChangeMamba & 2024 & 11.1 & 22.8 & 10.0 & 14.9 & 0.8 & 17.6 & 11.3 & & \\
%     Change3D & 2025 & 11.3 & 23.0 & 10.1 & 16.2 & 1.8 & 15.8 & 11.5 & & \\
%     CSDNet & 2026 & 12.4 & 24.1 & 11.8 & 17.0 & 1.0 & 19.0 & 12.5 & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Instance-level methods}} \\
%     Mask R-CNN & 2017 & 28.7 & 49.3 & 30.3 & 39.1 & 13.2 & 33.8 & 28.0 & 78.639 & 132.185 \\
%     Cascade Mask R-CNN & 2018 & 28.8 & 47.9 & 30.9 & 40.6 & 11.4 & 34.4 & 29.0 & 111.685 & 237.846 \\
%     Hybrid Task Cascade & 2019 & 30.8 & 51.4 & 32.8 & 41.1 & 14.7 & 36.7 & 31.0 & 114.573 & 241.324 \\
%     SOLOv2 & 2020 & 26.2 & 47.8 & 26.7 & 36.1 & 11.3 & 31.2 & - & 80.895 & 143.473 \\
%     SCNet & 2021 & 30.7 & 51.9 & 32.5 & 41.1 & 15.4 & 35.5 & 30.8 & 129.134 & 241.605 \\
%     Mask2Former & 2021 & 28.3 & 49.5 & 29.1 & 39.6 & 12.6 & 32.6 & 27.7 & 78.865 & 122.189 \\
%     FastInst & 2023 & 25.4 & 47.4 & 24.7 & 35.8 & 10.5 & 29.9 & 24.7 & 68.754 & 74.286 \\
%     ContourFormer & 2025 & 29.3 & 50.2 & 30.6 & 41.6 & 12.6 & 33.7 & 27.2 & 49.411 & 88.911 \\
%     D-FINE-seg & 2026 & 30.1 & 52.1 & 31.5 & 41.5 & 14.6 & 34.2 & 33.1 & 50.269 & 58.643 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{11}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
%     LAMIA-IBDA & -
%     & \textbf{33.5} & \textbf{55.4} & \textbf{36.1}
%     & \textbf{43.1} & \textbf{17.4} & \textbf{39.9}
%     & \textbf{34.0} & 149.228 & 327.779 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{table*}[t]
%   \centering
%   \caption{Instance-level building damage assessment on the xBD validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
%   \label{tab:textify_comparison_xbd}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}lc*{10}{c}@{}}
%     \toprule
%     \multirow{2}{*}[-3pt]{Method}
%     & \multirow{2}{*}[-3pt]{Year}
%     & \multicolumn{3}{c}{Mask AP$\uparrow$}
%     & \multicolumn{4}{c}{Class-wise mask AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Box AP$\uparrow$}
%     & \multirow{2}{*}[-3pt]{Params (M)}
%     & \multirow{2}{*}[-3pt]{GFLOPs} \\
%     \cmidrule(lr){3-5}\cmidrule(lr){6-9}
%     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$
%     & No damage & Minor & Major & Destroyed & & & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Pixel-level methods}} \\
%     % SNUNet & 2021 & 5.1 & 11.9 & 3.6 & 10.7 & 0.0 & 1.3 & 8.6 & 5.7 & & & \\
%     ChangeMamba & 2024 & 10.7 & 22.7 & 9.1 & 14.3 & 1.2 & 13.0 & 14.3 & 11.3 & & \\
%     Change3D & 2025 & 8.7 & 19.1 & 7.4 & 8.3 & 1.2 & 9.5 & 15.7 & 8.8 & & \\
%     CSDNet & 2026 & 11.8 & 24.3 & 10.7 & 17.4 & 2.4 & 11.7 & 15.8 & 12.5 &  & \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Instance-level methods}} \\
%     Mask R-CNN & 2017 & 28.6 & 51.1 & 30.2 & 35.0 & 17.3 & 30.4 & 31.9 & 28.3 & 55.136 & 132.206 \\
%     Cascade Mask R-CNN & 2018 & 29.4 & 50.9 & 31.7 & 35.4 & 17.4 & 31.3 & 33.5 & 30.0 & 88.181 & 237.906 \\
%     Hybrid Task Cascade & 2019 & 30.8 & 53.9 & 32.7 & 36.5 & 19.1 & 32.8 & 34.7 & 31.4 & 91.069 & 241.345 \\
%     SOLOv2 & 2020 & 26.0 & 50.3 & 25.1 & 31.1 & 14.7 & 29.2 & 29.0 & - & 57.391 & 143.491 \\
%     SCNet & 2021 & 30.1 & 53.0 & 31.7 & 35.9 & 18.0 & 32.8 & 33.8 & 30.9 & 105.630 & 241.626 \\
%     Mask2Former & 2021 & 29.4 & 53.4 & 30.3 & 35.2 & 18.0 & 30.9 & 33.6 & 29.0 & 55.357 & 122.191 \\
%     FastInst & 2023 & 25.0 & 48.6 & 24.4 & 31.3 & 12.7 & 26.7 & 29.4 & 23.8 & 45.248 & 74.286 \\
%     ContourFormer & 2025 & 29.8 & 54.7 & 30.7 & 37.1 & 18.5 & 30.6 & 33.0 & 30.0 & 39.364 & 88.913 \\
%     D-FINE-seg & 2026 & 30.1 & 55.6 & 30.5 & 37.2 & 18.4 & 31.2 & 33.6 & 33.9 & 40.223 & 58.645 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{12}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
%     % Textify-visual-baseline & 2026 & 33.1 & 56.4 & 35.8 & 38.6 & 21.6 & 35.3 & 36.8 & 33.7 & & & \\
%     LAMIA-IBDA & -
%     & \textbf{33.4} & \textbf{57.1} & \textbf{36.2}
%     & \textbf{39.0} & \textbf{21.7} & \textbf{35.7} & \textbf{37.3}
%     & \textbf{34.4} & 103.711 & 307.518 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/joplin.pdf}
%   \caption{Joplin}
%   \label{fig:joplin}
% \end{figure*}

% \subsection{Ablation Studies}

% \begin{table}[t]
%   \centering
%   \caption{Effect of text-guided fusion and text-based RoI classification.}
%   \label{tab:core_ablation}
%   \setlength{\tabcolsep}{2pt}
%   \renewcommand{\arraystretch}{1.08}
%   \begin{tabular}{@{}c*{5}{c}@{}}
%     \toprule
%     Fusion & Cls. & Mask AP$\uparrow$ & AP$_{50}$$\uparrow$ & AP$_{75}$$\uparrow$ & Box AP$\uparrow$\\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{6}{@{}l}{\textit{BRIGHT Dataset}} \\
%     $-$ & $-$ & 32.5 & 53.7 & 34.9 & 32.8 \\
%     $+$ & $-$ & 33.0 & 53.8 & 35.9 & 33.3 \\
%     $-$ & $+$ & 32.6 & 52.7 & 35.3 & 33.3 \\
%     $+$ & $+$ & 33.5 & 55.4 & 36.1 & 34.0 \\
%     \midrule
%     \rowcolor[HTML]{C0C0C0}
%     \multicolumn{6}{@{}l}{\textit{xBD Dataset}} \\
%     $-$ & $-$ & 32.7 & 55.8 & 35.6 & 33.7 \\
%     $+$ & $-$ & 33.0 & 56.7 & 35.6 & 33.9 \\
%     $-$ & $+$ & 32.9 & 56.6 & 35.7 & 33.7 \\
%     $+$ & $+$ & 33.4 & 57.1 & 36.2 & 34.4 \\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[t]
% \centering
% \caption{Sensitivity to the number of class descriptions per damage category. Prompts should be nested subsets so that wording changes are not confounded with prompt count.}
% \label{tab:prompt_count}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{2}{c}@{}}
% \toprule
% Prompts per class & Mask AP$\uparrow$ & Damaged/Minor AP$\uparrow$ \\
% \midrule
% \rowcolor[HTML]{C0C0C0}
% \multicolumn{3}{@{}l}{\textit{BRIGHT Dataset}} \\
% 2 & 32.4 & \\
% 4 & 32.2 & \\
% 6 & 32.9 & \\
% 8 & 33.5 & \\
% \midrule
% \rowcolor[HTML]{C0C0C0}
% \multicolumn{3}{@{}l}{\textit{xBD Dataset}} \\
% 2 & 33.0 & \\
% 4 & 33.4 & \\
% 6 & 33.0 & \\
% 8 & 32.5 & \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/n_prompt_ablation.pdf}
%   \caption{Overview of LAMIA-IBDA. The three highlighted modules are
%   Reliability-Guided Joint Attention, Overlap-Weighted Text Pooling, and
%   Contextual Prototype Classification. Case 1 and Case 2 illustrate different
%   visual-reliability regimes. The actual text-attention budget is determined
%   dynamically from the visual-reliability estimate during training; the shown
%   percentages are schematic. The auxiliary segmentation head, ground-truth
%   masks, and classifier-derived description distribution are used only for
%   training.}
%   \label{fig:n_prompt_ablation}
% \end{figure}

% \begin{table*}[t]
% \centering
% \caption{Sensitivity to the number of fusion encoder layers and local window size.}
% \label{tab:depth_window}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{4}{c}@{}}
% \toprule
% \multirow{2}{*}[-3pt]{Setting} & \multirow{2}{*}[-3pt]{Value} & \multicolumn{2}{c}{BRIGHT Dataset} & \multicolumn{2}{c}{xBD Dataset} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% & & Mask AP$\uparrow$ & Box AP$\uparrow$ & Mask AP$\uparrow$ & Box AP$\uparrow$ \\
% \midrule
% Encoder layers & 1 & 26.5 & 27.3 &   \\
% Encoder layers & 2 &  &  &   \\
% Encoder layers & 3 &  &  &  \\
% Encoder layers & 4 & 25.6 & 26.2 &  \\
% Tokenizer window size & 4 & 25.8 & 26.4 &   \\
% Tokenizer window size & 8 &  &  &  \\
% Tokenizer window size & 16 &  &   &  \\
% Attention supervision scales & stride 4 & 25.7 & 26.7 & & \\
% Attention supervision scales & stride 8 &  & & & \\
% Attention supervision scales & stride 4,8 & & & & \\
% Attention supervision scales & stride 4,8,16 & & & & \\
% Attention supervision scales & stride 4,8,16,32 & & & & \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \centering
% \caption{Sensitivity to the attention-supervision and instance-description alignment weights.}
% \label{tab:loss_weights}
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.08}
% \begin{tabular}{@{}lc*{4}{c}@{}}
% \toprule
% \multirow{2}{*}[-3pt]{Sweep} & \multirow{2}{*}[-3pt]{Value} & 
% \multicolumn{2}{c}{BRIGHT Dataset} & \multicolumn{2}{c}{xBD Dataset} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-6}
% & & Mask AP$\uparrow$ & Box AP$\uparrow$ & Mask AP$\uparrow$ & Box AP$\uparrow$ \\
% \midrule
% $\lambda_{\mathrm{attn}}$ & 0 &  &  & \\
% $\lambda_{\mathrm{attn}}$ & 0.05 &  &  &  \\
% $\lambda_{\mathrm{attn}}$ & 0.10 &  &  &  \\
% $\lambda_{\mathrm{attn}}$ & 0.20 &  &  & \\
% $\lambda_{\mathrm{align}}$ & 0 &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 0.5 &  &  &   \\
% $\lambda_{\mathrm{align}}$ & 1.0 &  &  &  \\
% $\lambda_{\mathrm{align}}$ & 2.0 &  &  & \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}[t]
%     \centering
%     \caption{Component-wise ablation of Textify. The full model is the reference row.}
%     \label{tab:component_ablation}
%     \setlength{\tabcolsep}{2pt}
%     \renewcommand{\arraystretch}{1.08}
%     \begin{tabular}{@{}lc*{6}{c}@{}}
%     \toprule
%     Variant & $\lambda_{\mathrm{attn}}$ & $\lambda_{\mathrm{align}}$ & Semantic probe & Nuisance text & Contextual prototype & Mask AP $\uparrow$ & $\Delta$AP \\
%     \midrule
%     Full & 0.1 & 1.0 & $+$ & $+$ & $+$ &  & \\
%     w/o text fusion &  &  &  &  &  &  &   \\
%     w/o text classification &  &  &  &  &  &  &  \\
%     w/o attention loss & 0 &  &  &  &  &  &    \\
%     w/o alignment loss &  & 0 &  &  &  &  &    \\
%     w/o semantic probe &  &  & 0 &  &  &  &   \\
%     w/o nuisance text &  &  &  & 0 &  &  &    \\
%     Static RoI prototype &  &  &  &  & 0 &  &    \\
%     w/o class-conditioned attention prompt &  &  &  &  &  &  &    \\
%     \bottomrule
%     \end{tabular}
% \end{table*}

% % \begin{table}[ht]
% % \centering
% % \caption{Accuracy and inference cost of the main Textify variants. Measure cost with the same input resolution and hardware.}
% % \label{tab:efficiency}
% % \scriptsize
% % \begin{tabular}{lcccccc}
% % \hline
% % Variant & Params (M) $\downarrow$ & FLOPs (G) $\downarrow$ & Peak memory (GB) $\downarrow$ & Latency (ms) $\downarrow$ & FPS $\uparrow$ & Mask AP $\uparrow$ \\
% % \hline
% % Visual &  &  &  &  &  &  \\
% % TGF &  &  &  &  &  &  \\
% % TGC &  &  &  &  &  &  \\
% % TGFC &  &  &  &  &  &  \\
% % \hline
% % \end{tabular}
% % \end{table}


% % \begin{table}[t]
% %   \centering
% %   \caption{num texts}
% %   \label{tab:isolation_n_texts}
% %   \setlength{\tabcolsep}{3pt}
% %   \renewcommand{\arraystretch}{1.08}
% %   \begin{tabular}{@{}lc*{2}{c}@{}}
% %     \toprule
% %     num texts & Mask AP & Box AP \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{3}{@{}l}{\textit{BRIGHT dataset}} \\
% %     2 & 32.0 & 32.6 \\
% %     4 & 32.0 & 32.3 \\
% %     6 & 31.5 & 31.8 \\
% %     8 & 32.1 & 32.5 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{3}{@{}l}{\textit{xBD dataset}} \\
% %     2 & 29.4 & 30.1 \\
% %     4 & 30.1 & 31.2 \\
% %     6 & 28.8 & 29.5 \\
% %     8 & 29.5 & 30.2 \\
% %     \bottomrule
% %   \end{tabular}
% % \end{table}

% % \begin{table}[t]
% %   \centering
% %   \caption{num fuse layers}
% %   \label{tab:isolation_n_layers}
% %   \setlength{\tabcolsep}{3pt}
% %   \renewcommand{\arraystretch}{1.08}
% %   \begin{tabular}{@{}lc*{2}{c}@{}}
% %     \toprule
% %     num fuse layers & Mask AP & Box AP \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{3}{@{}l}{\textit{BRIGHT dataset}} \\
% %     0 & 31.7 & 32.1 \\
% %     % 1 & 32.2 & 32.4 \\
% %     1 & 31.9 & 32.1 \\
% %     2 & 32.1 & 32.5 \\
% %     3 & 32.2 & 32.4 \\
% %     % 3 & 31.9 & 32.1 \\
% %     4 & 31.7 & 31.7 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{3}{@{}l}{\textit{xBD dataset}} \\
% %     0 &  &  \\
% %     1 &  &  \\
% %     2 &  &  \\
% %     3 &  &  \\
% %     4 &  &  \\
% %     \bottomrule
% %   \end{tabular}
% % \end{table}

% % \begin{table*}[t]
% %   \centering
% %   \caption{Instance-level building damage assessment on the BRIGHT validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
% %   \label{tab:textify_comparison_bright}
% %   \normalsize
% %   \setlength{\tabcolsep}{3pt}
% %   \renewcommand{\arraystretch}{1.08}
% %   \begin{tabular}{@{}lc*{7}{c}@{}}
% %     \toprule
% %     \multirow{2}{*}[-3pt]{Method} & \multirow{2}{*}[-3pt]{Year} & \multicolumn{3}{c}{Mask AP ($\uparrow$)} & \multicolumn{3}{c}{Class-wise mask AP ($\uparrow$)} & \multirow{2}{*}[-3pt]{Box AP ($\uparrow$)} \\
% %     \cmidrule(lr){3-5}\cmidrule(lr){6-8}
% %     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$ & Intact & Damaged & Destroyed & \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{9}{@{}l}{\textit{Pixel-level methods}} \\
% %     ChangeFormer & 2022 & 11.1 & 22.8 & 10.0 & 14.9 & 0.8 & 17.6 & 11.3 \\
% %     Changer & 2023 & 11.3 & 23.0 & 10.1 & 16.2 & 1.8 & 15.8 & 11.5 \\
% %     ChangeMamba & 2024 &  &  &  &  &  &  &  \\
% %     ChangeCD & 2025 &  &  &  &  &  &  &  \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{9}{@{}l}{\textit{Instance-level methods}} \\
% %     Mask R-CNN & 2017 & 28.7 & 49.3 & 30.3 & 39.1 & 13.2 & 33.8 & 28.0 \\
% %     Cascade Mask R-CNN & 2018 & 28.8 & 47.9 & 30.9 & 40.6 & 11.4 & 34.4 & 29.0 \\
% %     Hybrid Task Cascade & 2019 & 30.8 & 51.4 & 32.8 & 41.1 & 14.7 & 36.7 & 31.0 \\
% %     SOLOv2 & 2020 & 26.2 & 47.8 & 26.7 & 36.1 & 11.3 & 31.2 & - \\
% %     SCNet & 2021 & 30.7 & 51.9 & 32.5 & 41.1 & 15.4 & 35.5 & 30.8 \\
% %     Mask2Former & 2021 & 28.3 & 49.5 & 29.1 & 39.6 & 12.6 & 32.6 & 27.7 \\
% %     FastInst & 2023 & 25.4 & 47.4 & 24.7 & 35.8 & 10.5 & 29.9 & 24.7 \\
% %     ContourFormer & 2025 & 29.3 & 50.2 & 30.6 & 41.6 & 12.6 & 33.7 & 27.2 \\
% %     D-FINE-seg & 2026 & 30.1 & 52.1 & 31.5 & 41.5 & 14.6 & 34.2 & 33.1 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{9}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
% %     LAMIA-IBDA & 2026 & \textbf{33.5} & \textbf{55.4} & \textbf{36.1} & \textbf{43.1} & \textbf{17.4} & \textbf{39.9} & \textbf{34.0} \\
% %     \bottomrule
% %   \end{tabular}
% % \end{table*}

% % \begin{table*}[t]
% %   \centering
% %   \caption{Instance-level building damage assessment on the xBD validation set. All AP values are on a 0--100 scale ($\uparrow$). Bold indicates the highest reported value in each column.}
% %   \label{tab:textify_comparison_xbd}
% %   \setlength{\tabcolsep}{3pt}
% %   \renewcommand{\arraystretch}{1.08}
% %   \begin{tabular}{@{}lc*{8}{c}@{}}
% %     \toprule
% %     \multirow{2}{*}[-3pt]{Method} & \multirow{2}{*}[-3pt]{Year} & \multicolumn{3}{c}{Mask AP ($\uparrow$)} & \multicolumn{4}{c}{Class-wise mask AP ($\uparrow$)} & \multirow{2}{*}[-3pt]{Box AP ($\uparrow$)} \\
% %     \cmidrule(lr){3-5}\cmidrule(lr){6-9}
% %     & & $\mathrm{AP}$ & $\mathrm{AP}_{50}$ & $\mathrm{AP}_{75}$ & No damage & Minor & Major & Destroyed & \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{10}{@{}l}{\textit{Pixel-level methods}} \\
% %     % SNUNet & 2021 & 5.1 & 11.9 & 3.6 & 10.7 & 0.0 & 1.3 & 8.6 & 5.7 \\
% %     ChangeFormer & 2022 &  &  &  &  &  &  &  &  \\
% %     Changer & 2023 &  &  &  &  &  &  &  &  \\
% %     ChangeMamba & 2024 \\
% %     ChangeCD & 2025 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{10}{@{}l}{\textit{Instance-level methods}} \\
% %     Mask R-CNN & 2017 & 28.6 & 51.1 & 30.2 & 35.0 & 17.3 & 30.4 & 31.9 & 28.3 \\
% %     Cascade Mask R-CNN & 2018 & 29.4 & 50.9 & 31.7 & 35.4 & 17.4 & 31.3 & 33.5 & 30.0 \\
% %     Hybrid Task Cascade & 2019 & 30.8 & 53.9 & 32.7 & 36.5 & 19.1 & 32.8 & 34.7 & 31.4 \\
% %     SOLOv2 & 2020 & 26.0 & 50.3 & 25.1 & 31.1 & 14.7 & 29.2 & 29.0 & - \\
% %     SCNet & 2021 & 30.1 & 53.0 & 31.7 & 35.9 & 18.0 & 32.8 & 33.8 & 30.9 \\
% %     Mask2Former & 2021 & 29.4 & 53.4 & 30.3 & 35.2 & 18.0 & 30.9 & 33.6 & 29.0 \\
% %     FastInst & 2023 & 25.0 & 48.6 & 24.4 & 31.3 & 12.7 & 26.7 & 29.4 & 23.8 \\
% %     ContourFormer & 2025 &  &  &  &  &  &  &  &  \\
% %     D-FINE-seg & 2026 & 30.1 & 55.6 & 30.5 & 37.2 & 18.4 & 31.2 & 33.6 & 33.9 \\
% %     \midrule
% %     \rowcolor[HTML]{C0C0C0}
% %     \multicolumn{10}{@{}l}{\textit{Text-guided instance-level method (Ours)}} \\
% %     % Textify-visual-baseline & 2026 & 33.1 & 56.4 & 35.8 & 38.6 & 21.6 & 35.3 & 36.8 & 33.7 \\
% %     LAMIA-IBDA & 2026 & \textbf{33.4} & \textbf{57.1} & \textbf{36.2} & \textbf{39.0} & \textbf{21.7} & \textbf{35.7} & \textbf{37.3} & \textbf{34.4} \\
% %     \bottomrule
% %   \end{tabular}
% % \end{table*}

% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\linewidth]{fig/ablations.pdf}
%   \caption{Ablation studies of LAMIA-IBDA on BRIGHT and xBD. Module gains are relative to the visual-only baseline; text-representation changes are relative to the full model and are evaluated without retraining. The remaining panels report absolute mask AP.}
%   \label{fig:ablations}
% \end{figure*}

% \section{Ablation Studies}
% \label{sec:ablations}

% \subsection{Experimental protocol}
% All ablation experiments use the same data splits, visual backbone, FPN,
% HTC instance head, training schedule, and four-quadrant inference protocol
% as the main experiments. We report mask AP, $\mathrm{AP}_{50}$, and
% $\mathrm{AP}_{75}$ on BRIGHT and xBD. Unless otherwise stated, each
% architecture or loss configuration is trained from scratch under the same
% protocol. The inference-time ablations in
% Table~\ref{tab:inference_ablations} instead evaluate a fixed trained model
% without retraining.

% \subsection{Text-guided modules}
% Table~\ref{tab:core_ablation} separates the effects of Adaptive
% Text-Visual Alignment and contextual text-prototype classification. On
% BRIGHT, text-guided fusion alone improves mask AP from 32.5 to 33.0,
% whereas text-based classification alone gives 32.6. Combining both modules
% reaches 33.5 AP, with consistent gains at both $\mathrm{AP}_{50}$ and
% $\mathrm{AP}_{75}$. The same trend appears on xBD, where the complete model
% achieves 33.4 AP compared with 32.7 for the visual-only baseline. These
% results show that semantic fusion and prototype classification provide
% complementary benefits.

% \subsection{Token composition}
% Table~\ref{tab:attn_ablation} evaluates which token groups should
% participate in joint attention. Using only change tokens yields 29.9 AP on
% BRIGHT and 30.8 AP on xBD. Adding visual tokens provides limited additional
% information, while adding text tokens gives a larger improvement, reaching
% 32.9 and 32.6 AP, respectively. Using all three token groups achieves the
% best results, 33.5 AP on BRIGHT and 33.4 AP on xBD. This result confirms
% that change, visual, and text tokens provide complementary evidence for
% bi-temporal damage reasoning.

% \subsection{Contextual text representations}
% Table~\ref{tab:inference_ablations} evaluates the role of image-conditioned
% text states and semantic prompt assignment. Removing text updates reduces
% mask AP from 33.5 to 29.6 on BRIGHT and from 33.4 to 31.0 on xBD. Using
% static text only for the classifier produces similar drops, showing that
% both fusion-time text updating and classification-time contextualization
% are important. Shuffling prompt labels or replacing text with random
% vectors causes substantially larger degradation, which verifies that the
% improvements depend on meaningful class semantics rather than on an
% additional arbitrary feature branch.

% \subsection{Description number and allocation}
% Table~\ref{tab:prompt_count} studies the number of descriptions assigned
% to each damage category. On BRIGHT, increasing the number of descriptions
% from a single class name to $(4,8,6)$ improves mask AP from 30.8 to 33.5.
% On xBD, the best overall AP is obtained with $(4,8,8,6)$, while the
% $(4,8,8,4)$ configuration gives the highest $\mathrm{AP}_{75}$. These
% results show that complementary descriptions are more useful than a single
% class name and that uniform prompt allocation is not optimal. The final
% configurations therefore use $(4,8,6)$ for BRIGHT and $(4,8,8,6)$ for xBD.

% \subsection{Auxiliary loss weights}
% Table~\ref{tab:loss_weights} examines the sensitivity to the two auxiliary
% loss weights. When $\lambda_{\mathrm{ATVA}}$ increases from 0 to 0.1,
% mask AP improves from 32.7 to 33.5 on BRIGHT and from 32.6 to 33.4 on xBD.
% A further increase to 0.2 slightly reduces performance. Similarly,
% $\lambda_{\mathrm{align}}=1.0$ gives the best results on both datasets,
% whereas removing the alignment loss or assigning it an excessive weight
% leads to lower AP. We therefore use
% $\lambda_{\mathrm{ATVA}}=0.1$ and
% $\lambda_{\mathrm{align}}=1.0$ in the final model.
